Designing Transportable Experiments

We consider the problem of designing a randomized experiment on a source population to estimate the Average Treatment Effect (ATE) on a target population. We propose a novel approach which explicitly considers the target when designing the experiment on the source. Under the covariate shift assumption, we design an unbiased importance-weighted estimator for the target population's ATE. To reduce the variance of our estimator, we design a covariate balance condition (Target Balance) between the treatment and control groups based on the target population. We show that Target Balance achieves a higher variance reduction asymptotically than methods that do not consider the target population during the design phase. Our experiments illustrate that Target Balance reduces the variance even for small sample sizes.

==> 1d.tex <==
\subsection{Variance - General Case}
We assume that $n_1 = n_0 = n/2$, $X \in R^d$ where $d=1$, and
\begin{align}
    Y^{A_i}_i &= f(X_i) + A_i * g(X_i) + \epsilon_i
\end{align}
where $\epsilon_i \sim Norm(0,1) $.

Define 
\begin{align}
    T_i &= f(X_i) + g(X_i)/2 + \epsilon_i 
\end{align}

Conditioning on $\X = \x$, we can do linear regression on $\T$ and $\x$ and obtain: 
\begin{align}
    T_i = \beta^T x_i + R_i 
\end{align}
where $R_i$'s are iid normal. 
We assume that $T_i$ is linear in term of $x_i$, and therefore $R_i$ is $Norm(0,1)$. \my{ Relax this assumption later for non-linearity}. 

Let $\varphi(\X, \A) = \norm{ \frac{2}{n} \left( \sum_{i: A_i = 1} w_i X_i - \sum_{i: A_i = 0} w_i  X_i\right) } < a$. First we note that:
\begin{align}
    \varphi(\X, \A) = \varphi(\X, 1-\A)
\end{align}
which satisfies the condition in Lemma~\ref{lem:unbiased2}. 

Let $ Q = \frac{p_T(X)}{p_S(X)} X$.
\begin{align}
 %   \EE_S(Z) &= \EE_S \left(\frac{p_T(X)}{p_S(X)} \epsilon \right) = \EE_T( \epsilon) = 0 \\
    \EE_S(Q) &= \EE_S \left(\frac{p_T(X)}{p_S(X)} X\right) = \EE_T(X)  
\end{align}

\begin{align}
    \var_S(Q) = \var_S\left(\frac{p_T(X)}{p_S(X)} X \right) 
    &= \EE_S \left(\frac{p_T(X)}{p_S(X)} X  \right) ^2  - \left( \EE_S \frac{p_T(X)}{p_S(X)} X \right) ^2 \\
    &= \EE_T \left [\frac{p_T(X)}{p_S(X)} (X)^2\right ] - (\EE_T X)^2 \\
    &= \EE_T \left [\frac{p_T(X)}{p_S(X)} (X)^2\right ] - (\EE_T X)^2
\end{align}
% \begin{align}
%      \var_S(Z) = \var_S\left(\frac{p_T(X)}{p_S(X)} \epsilon \right) 
%     &= \EE_S \left(\frac{p_T(X)}{p_S(X)} \epsilon \right) ^2  - \left( \EE_S \frac{p_T(X)}{p_S(X)} \epsilon \right) ^2 \\
%     &= \EE_T \left [\frac{p_T(X)}{p_S(X)} ({\epsilon})^2\right ] - (\EE_T \epsilon^0)^2 \\
%     &= \EE_T \left [\frac{p_T(X)}{p_S(X)} ({\epsilon})^2\right ] \text{ because } \EE_T \epsilon = 0\\
%     &= \EE_T \left [\frac{p_T(X)}{p_S(X)} \right] \EE[ {\epsilon}^2 ] \text{because  $\frac{p_T(X)}{p_S(X)}$ and $\epsilon$ are independent} \\
%     &= \EE_T \left [\frac{p_T(X)}{p_S(X)} \right] \text{ because } \EE[ \epsilon^2 ]=1
% \end{align}
% \begin{align}
%     cov_S(Q,R) &= \EE_S[QR] - \EE_S[Q] \EE_S[R] \\
%     &= \EE_S\left[ \frac{p_T(X)^2}{p_S(X)^2} X \epsilon^0\right] - 0 
% \end{align}


First we analyze the variance of $\hat{\tau}$ without the balance condition:
\begin{align}
&\var_S(\hat{\tau} | \X= \mathbf{x}) \\
&= \frac{2}{n}\var_S(\frac{1}{n_1} \sum_{i=1}^n w_iA_i Y^1_i - \frac{1}{n_0} \sum_{i=1}^n w_i (1-A_i) Y^0_i | \X= \mathbf{x}) \\
&= \frac{2}{n}\var_S( \sum_{i: A_i = 1} w_i Y^1_i - \sum_{i: A_i = 0} w_i  Y^0_i | \X= \mathbf{x}) \\
&= \frac{2}{n}\var_S( \sum_{i: A_i = 1} w_i T_i - \sum_{i: A_i = 0} w_i  T_i + \sum_{i=1}^n  w_i \frac{g(x_i)}{2} \bigg| \X= \mathbf{x}) \\
&= \frac{2}{n}\var_S( \sum_{i: A_i = 1} w_i T_i - \sum_{i: A_i = 0} w_i  T_i | \X= \mathbf{x}) \\
&= \frac{2}{n}\var_S( \sum_{i: A_i = 1} w_i \beta^T x_i - \sum_{i: A_i = 0} w_i \beta^T  x_i \big| \X= \mathbf{x}) \label{eq:term1}\\&+ \frac{2}{n}\var_S( \sum_{i: A_i = 1} w_iR_i - \sum_{i: A_i = 0} w_i  R_i \big| \X= \mathbf{x}) \label{eq:term2}%\\&+ \frac{8}{n} \sum_{i = 1}^n \sum_{j=1}^n w_i w_j Cov(A_i, A_j)  \EE[ R_j \big |\X = \x]
\end{align}

The last equality is because conditioning on $\X = \mathbf{x}$, we will show that if $\EE[R_i| \X = x] = 0$ then
\begin{align}
    &Cov \left( \sum_{i: A_i = 1} w_i x_i - \sum_{i: A_i = 0} w_i  x_i , \sum_{i: A_i = 1} w_i R_i - \sum_{i: A_i = 0} w_i  R_i  \bigg| \X = \x \right ) = 0
\end{align}  
We have:
\begin{align}
    &Cov \left( \sum_{i: A_i = 1} w_i x_i - \sum_{i: A_i = 0} w_i  x_i ,  \sum_{i: A_i = 1} w_i R_i - \sum_{i: A_i = 0} w_i  R_i  \bigg| \X = \x \right ) \\
    &= Cov \left( \sum_{i=1}^n A_i w_i x_i - \sum_{i=1}^n (1-A_i) w_i  x_i ,\sum_{i=1}^n A_i w_i R_i - \sum_{i=1}^n (1-A_i) w_i  R_i \bigg| \X = \x \right )  \\
    &= Cov \left( \sum_{i=1}^n 2 A_i w_i x_i - \sum_{i=1}^n  w_i  x_i ,  \sum_{i=1}^n (2 A_i -1) w_i R_i  \bigg| \X = \x \right ) \\
    &= Cov \left( \sum_{i=1}^n 2 A_i w_i x_i ,\sum_{i=1}^n (2 A_i-1)  w_i R_i \big| \X = \x \right ) \\
    &= \sum_{i = 1}^n \sum_{j=1}^n w_i w_j Cov \left( 2A_i, (2A_j -1) R_j \big |\X = \x \right)  
\end{align}
where
\begin{align}
    &Cov \left( 2A_i, (2A_j -1) R_j \big |\X = \x \right)  \\
     & = \EE[2A_i (2A_j -1) R_j \big |\X = \x] - \EE[2A_i] \EE [(2A_j -1) R_j \big |\X = \x ] \\
     & = \EE[2A_i (2A_j -1) ] \EE[ R_j \big |\X = \x] - \EE[2A_i] \EE [(2A_j -1)] \EE[ R_j \big |\X = \x] \text{ because $R_j$ and $A_i, A_j$ are independent} \\
      & = Cov(2A_i, 2A_j -1)  \EE[ R_j \big |\X = \x] \\
       & = 4 Cov(A_i, A_j)  \EE[ R_j \big |\X = \x] \\ 
       &= 0 \text{ because } \EE[ R_j \big |\X = \x] = 0 
 \end{align}

For the first term in Eq~\ref{eq:term1}, by finite population CLT \citep{li2016general}, when $n$ is large
$\frac{2}{n}( \sum_{i: A_i = 1} w_i X_i - \sum_{i: A_i = 0} w_i  X_i ) | \X= \mathbf{x}$ converges in distribution to $Norm(\EE_S[Q] , \frac{\var_S(Q)}{n}) = Norm(\EE_T[X] , \frac{\var_S(Q)}{n}) $ \my{Is this correct?}

For the 2nd term in Eq.~\ref{eq:term2}:
\begin{align}
&\frac{2}{n}\var( \sum_{i: A_i = 1} W_i R_i - \sum_{i: A_i = 0} W_i  R_i  | \X= \mathbf{x}) \\
&=\frac{2}{n}\var( \sum_{i: A_i = 1} w_i R_i - \sum_{i: A_i = 0} w_i  R_i ) \\
%&=\frac{2}{n}\var( 2 \sum_{i: A_i = 1} w_i R_i - \sum_{i=1}^n w_i  R_i ) \\
&=\frac{2}{n}\left(\var( \EE[  \sum_{i: A_i = 1} w_i R_i - \sum_{i: A_i = 0} w_i  R_i | \A] ) + \EE[ \var(  \sum_{i: A_i = 1} w_i R_i - \sum_{i: A_i = 0} w_i  R_i | \A) ]\right) \\
&=\frac{2}{n}\left(\var(0) + \EE[   \sum_{i=1}^n w_i  ]\right) \text{ because $R_i$ is $Norm(0,1)$} \\
&= \frac{2}{n} \left (\sum_{i=1}^n w_i  \right)
\end{align}



  Therefore when $n$ is large: 
\begin{align}
&\var_S(\hat{\tau}| \X= \mathbf{x}) = \frac{ 2\var_S(Q) }{n} + \frac{2 \sum_{i=1}^n w_i}{n}%+ \frac{8}{n} \sum_{i = 1}^n \sum_{j=1}^n w_i w_j Cov(A_i, A_j)  \EE[ R_j \big |\X = \x]
\end{align}



Now we analyze the variance of $\hat{\tau}$ with the balance condition:
\begin{align}
&\var_S(\hat{\tau} | \X= \mathbf{x}, \varphi(\X, \A) = 1) \\
&= \frac{2}{n}\var_S( \sum_{i: A_i = 1} w_i T_i - \sum_{i: A_i = 0} w_i  T_i | \X= \mathbf{x}, , \varphi(\X, \A) = 1) \\
&= \frac{2}{n}\var_S( \sum_{i: A_i = 1} w_i \beta^T x_i - \sum_{i: A_i = 0} w_i \beta^T  x_i \big| \X= \x, , \varphi(\X, \A) = 1) \label{eq:term1_balance}\\
&+ \frac{2}{n}\var_S( \sum_{i: A_i = 1} w_iR_i - \sum_{i: A_i = 0} w_i  R_i \big| \X= \mathbf{x}, , \varphi(\X, \A) = 1) \label{eq:term2_baalnce}%\\&+ \frac{8}{n} \sum_{i = 1}^n \sum_{j=1}^n w_i w_j Cov(A_i, A_j)  \EE[ R_j \big |\X = \x]
\end{align}
The last equality is because conditioning on $\X = \mathbf{x}$ and $\varphi(\X, \A) =1$, we will show that if $\EE[R_i| \X = x] = 0$ then
\begin{align}
\label{eq:uncorrelated}
    &Cov \left( \sum_{i: A_i = 1} w_i x_i - \sum_{i: A_i = 0} w_i  x_i  , \sum_{i: A_i = 1} w_i R_i - \sum_{i: A_i = 0} w_i  R_i \bigg| \X = \x , \varphi(\X, \A) =1 \right ) = 0
\end{align}  
We have: 
\begin{align}
    &Cov \left( \sum_{i: A_i = 1} w_i x_i - \sum_{i: A_i = 0} w_i  x_i , \sum_{i: A_i = 1} w_i R_i - \sum_{i: A_i = 0} w_i  R_i  \bigg| \X = \x , \varphi(\X, \A) =1 \right ) \\
      &=Cov \left (\sum_{i=1}^n w_i A_i x_i - \sum_{i=1}^n w_i (1-A_i)  x_i  , \sum_{i=1}^n w_i A_i R_i - \sum_{i=1}^n w_i (1-A_i) R_i  \bigg| \X = \x , \varphi(\X, \A) =1 \right ) \\
      &=Cov \left( \sum_{i=1}^n w_i (2A_i -1) x_i  ,  \sum_{i=1}^n w_i (2A_i -1)R_i  \bigg| \X = \x , \varphi(\X, \A) =1 \right ) \\
      &=Cov \left( \sum_{i=1}^n 2 w_i A_i  x_i  ,  \sum_{i=1}^n w_i (2A_i -1)R_i  \bigg| \X = \x , \varphi(\X, \A) =1 \right ) \\
    &= \sum_{i = 1}^n \sum_{j=1}^n w_i w_j Cov \left( 2A_i, (2A_j -1) R_j \bigg |\X = \x , \varphi(\X, \A) = 1\right)  
\end{align} 
where
\begin{align}
    &Cov \left( 2A_i, (2A_j -1) R_j \big |\X = \x, \varphi(\X, \A) = 1 \right)  \\
     & = \EE[2A_i (2A_j -1) R_j \big |\X = \x, \varphi(\X, \A) = 1] - \EE[2A_i | \varphi(\X, \A) = 1] \cdot \EE [(2A_j -1) R_j \big |\X = \x, \varphi(\X, \A) = 1 ] \\
     & = \EE[2A_i (2A_j -1) | \varphi(\X, \A) = 1] \cdot \EE[ R_j \big |\X = \x, \varphi(\X, \A) = 1] \\ &- \EE[2A_i | \varphi(\X, \A) = 1] \cdot \EE [(2A_j -1) | \varphi(\X, \A) = 1] \cdot \EE[ R_j \big |\X = \x, \varphi(\X, \A) = 1] \\ &\text{ because $R_j$ and $A_j$, $R_j$ and $2A_i(2A_j -1)$ are independent conditioning on }\X = \x, \varphi(\X, \A) = 1 \\
      & = Cov(2A_i, 2A_j -1 | \varphi(\X, \A) = 1)  \EE[ R_j \big |\X = \x] \\
       & = 4 Cov(A_i, A_j)  \EE[ R_j \big |\X = \x] \\ 
       &= 0 \text{ because } \EE[ R_j \big |\X = \x] = 0 
 \end{align}
 
We analyze the first term in Eq.~\ref{eq:term1_balance}. Since $\frac{2}{n}( \sum_{i: A_i = 1} w_i X_i - \sum_{i: A_i = 0} w_i  X_i \big| \X= \mathbf{x}$ is approximately $Norm(0, \frac{\var_S(Q)}{n})$ for large $n$, $\frac{2}{n}( \sum_{i: A_i = 1} w_i X_i - \sum_{i: A_i = 0} w_i  X_i \big| \X= \mathbf{x}, \varphi(\X, \A) = 1$ is a truncated Gaussian. Let $V \sim Norm(0, \sigma^2)$, then $\var(V | \norm{V} < a)$ is: 
\begin{align}
    \sigma^2 \left[ 1- \frac{2\sqrt{a} g(\sqrt{a})}{F(\sqrt{a}/\sigma) - F(-\sqrt{a}/{\sigma})} \right]
\end{align}
where $g(x) = \frac{1}{\sqrt{2\pi}} exp(-0.5x^2)$ and $F(x)$ is the CDF of the standard normal distribution. Therefore the first term equal to:
\begin{align}
     \frac{2\var_S(Q)}{n} \left[ 1- \frac{2\sqrt{a} g(\sqrt{a})}{F(\sqrt{a}/\sigma) - F(-\sqrt{a}/{\sigma})} \right]
\end{align}

Now we analyze the 2nd term in Eq.~\ref{eq:term2_baalnce}. 

\begin{align}
    &\frac{2}{n}\var( \sum_{i: A_i = 1} w_i R_i - \sum_{i: A_i = 0} w_i  R_i \big| \X = \x, \varphi(\X, \A) = 1) \\
     &=\frac{2}{n} \EE \left[ \left(\sum_{i: A_i = 1} w_i R_i - \sum_{i: A_i = 0} w_i  R_i \right)^2\bigg| \X = \x, \varphi(\X, \A) = 1 \right] - \frac{2}{n} \left(\EE \left[ \sum_{i: A_i = 1} w_i R_i - \sum_{i: A_i = 0} w_i  R_i \bigg| \X = \x, \varphi(\X, \A) = 1) \right] \right)^2 \\
      &=\frac{2}{n}\EE \left[ \left(\sum_{i: A_i = 1} w_i R_i - \sum_{i: A_i = 0} w_i  R_i \right)^2\bigg| \X = \x, \varphi(\X, \A) = 1 \right] - 0 \text{ because } \EE[R_i | \X = \x, \varphi(\X, \A) = 1]=0\\
     &=\frac{2}{n}\EE \left[ \left(\sum_{i=1}^n w_i A_i R_i  -  \sum_{i=1}^n w_i (1-A_i) R_i \right)^2 \bigg| \X = \x, \varphi(\X, \A) = 1 \right] \\
        &=\frac{2}{n}\EE \left[ \left(\sum_{i=1}^n w_i (2A_i -1) R_i   \right)^2 \bigg| \X = \x, \varphi(\X, \A) = 1 \right] \\
         &=\frac{2}{n}\EE \left[ \sum_{i=1}^n \sum_{j=1}^n w_i w_j (2 A_i -1) (2A_j -1 ) R_i R_j  \bigg| \X = \x, \varphi(\X, \A) = 1 \right] \\
           &=\frac{2}{n}\EE \left[ \sum_{i=1}^n w_i^2 (2 A_i -1)^2  R_i^2 \bigg| \X = \x, \varphi(\X, \A) = 1 \right] \text{ because when $i\neq j$ we can factor out $\EE[R_j | \X = \x, \varphi(\X,\A]$ which is $0$}\\
            &=\frac{2}{n}\EE \left[ \sum_{i=1}^n w_i^2   R_i^2 \bigg| \X = \x, \varphi(\X, \A) = 1 \right] \text{ because $(2 A_i -1)^2=1$ for all $A_i$}\\
            &=\frac{2}{n}\sum_{i=1}^n \EE \left[  w_i^2   R_i^2 \right] \\
            &=\frac{2}{n}\sum_{i=1}^n \left (\EE \left[  w_i^2   R_i^2 \right] - \left (\EE \left[  w_i   R_i \right] \right)^2 \right)\\
            &=\frac{2}{n}\sum_{i=1}^n \var(w_i R_i) \\
    &= \frac{2 \sum_{i=1}^n w_i}{n}
\end{align}

% Conditioning on $\X = \x$,  $U = \sum_{i: A_i = 1} w_i X_i - \sum_{i: A_i = 0} w_i X_i$ and $V = \sum_{i: A_i = 1} w_i R_i - \sum_{i: A_i = 0} w_i  R_i$ are uncorrelated from Eq.~\ref{eq:uncorrelated}. We will show that conditioning on $\X =\x$, they are  bivariate Gaussian by showing that conditioning on $\X=\x$, $aU + bV$ is Gaussian for any constant $a,b$:
% \begin{align}
%     &aU + bV \\
%     &= a \left ( \sum_{i: A_i = 1} w_i x_i - \sum_{i: A_i = 0} w_i x_i \right) + b \left (\sum_{i: A_i = 1} w_i R_i - \sum_{i: A_i = 0} w_i  R_i \right ) \\
%     & = \sum_{i: A_i = 1} w_i (a x_i - b R_i ) - \sum_{i: A_i = 0} w_i (a x_i - b R_i) \label{eq:bivariate}
% \end{align}
% Let $W =  \frac{p_T(X)}{p_S(X)} (a X - b R)$ where $R$ is iid with $R_i$. By finite CLT, Eq.~\ref{eq:bivariate} will converge in distribution to $Norm(\EE_S[W], n \var_S(W))$. 

% Since $U$ and $V$ are uncorrelated and bivariate Gaussian conditioning on $\X = \x$, they are independent conditioning on $\X = \x$\my{is it correct?}.  Therefore $\sum_{i: A_i = 1} w_i R_i - \sum_{i: A_i = 0} w_i  R_i$ and $\varphi(\X, \A)$ are independent conditioning on $\X = \x$. 
% \begin{align}
%     &\frac{2}{n}\var( \sum_{i: A_i = 1} w_i R_i - \sum_{i: A_i = 0} w_i  R_i \big| \X = \x, \varphi(\X, \A) = 1) \\
%     = & \frac{2}{n}\var( \sum_{i: A_i = 1} w_i R_i - \sum_{i: A_i = 0} w_i  R_i \big| \X = \x)  \\
%     =& \frac{2 \sum_{i=1}^n w_i}{n}
% \end{align}


Summing up the first term and the second term:
\begin{align}
     &\var_S(\hat{\tau}| \X= \mathbf{x}, \varphi(\X, \A) = 1) \\
     &=2\frac{\var_S(Q)}{n} \left[ 1- \frac{2\sqrt{a} g(\sqrt{a})}{F(\sqrt{a}/\sigma) - F(-\sqrt{a}/{\sigma})} \right] + \frac{2 \sum_{i=1}^n w_i}{n}
\end{align}
Recall that: 
\begin{align}
&\var_S(\hat{\tau}| \X= \mathbf{x}) = \frac{ 2\var_S(Q)  }{n}+  \frac{2 \sum_{i=1}^n w_i}{n}
\end{align}


==> analysis.tex <==
\section{Analysis}
\label{sec:analysis}
% We propose using the importance weighted estimator to estimate the ATE in the target distribution. 
% \begin{definition}[Importance-weighted Estimator]
% \label{def:weighted_estimator}
% We define the importance weighted estimator $\hat{\tau}^S_Y$ from the source distribution:
% \begin{align*}
%     \hat{\tau}^S_Y %&= \frac{1}{n_1} \sum_{i=1}^n W_iA_i Y^{A_i}_i - \frac{1}{n_0} \sum_{i=1}^n W_i (1-A_i) Y^{A_i}_i \\
%     %  &= \frac{1}{n_1} \sum_{i=1}^n \frac{p_T(Y_i|X_i) p_T(X_i)}{p_S(Y_i | X_i) p_S(X_i)}A_i Y^{A_i}_i - \frac{1}{n_0} \sum_{i=1}^n \frac{p_T(Y_i|X_i) p_T(X_i)}{p_S(Y_i | X_i) p_S(X_i)} (1-A_i) Y^{A_i}_i \text{ because } p_S(Y_i | X_i ) = p_T(Y_i | X_i) \\
%     &= \frac{1}{n_1} \sum_{i=1}^n W_iA_i Y^1_i - \frac{1}{n_0} \sum_{i=1}^n W_i (1-A_i) Y^0_i
% \end{align*}
% where $W_i  =  \frac{p_T(X_i)}{p_S(X_i)} $ and $w_i  = \frac{p_T(x_i)}{p_S(x_i)} $.
% \end{definition}
In Section~\ref{sec:expectation} we show that the importance-weighted estimator in Definition~\ref{def:weighted_estimator} is unbiased when the balance condition $\rho$ is symmetric with respect to $\A$: $\rho(\X, \A) = \rho(\X, 1- \A)$. In Section~\ref{sec:variance} we define a balance condition (Target Balance) that satisfies the symmetry condition and show that using Target Balance will reduce the variance of the importance-weighted estimator. 


\input{expectation}

\subsection{Variance}
\label{sec:variance}
In this section we specify our Mahalanobis-based balance criteria (Target Balance) in Definition~\ref{def:balance}.  Theorem~\ref{thm:variance_with_balance} shows that we can achieve variance reduction under Target Balance in the linear model if the weighted covariates' mean is a multivariate normal \footnote{Due to the finite central limit theorem, the weighted covariates' mean is asymptotically normal.}. In Theorem~\ref{thm:optimality}, we show that for a rejection threshold $\alpha$, our balance criteria achieves the largest variance reduction. 

Without loss of generalization we assume that $X$ contains a bias term $X_1 = 1$. 
Define 
\begin{align*}
    T = \frac{Y^1 + Y^0}{2},
\end{align*}
which plays an important role in our analysis. Using the same convention as in Section~\ref{sec:problem_setting}, let $\T$ denote the $n \times 1$ vector of random variables $T_1, ..., T_n$ and $\ttt$ denote a particular value taken by $\T$. 

We consider the linear model where:
\begin{align*}
    T = \beta^T X + R.
\end{align*}
where $\EE[R] = 0$ and $R$ is independent of $X$. Let $\sigma^2_R = Var(R) = \EE[R^2].$ \anup{Probably give a concrete example for $Y^1 (X) = \cdot$ and $Y^2(X) = \cdot$ which satisfies this condition on $T.$}

For notation convenience we define $Z_i = 2A_i - 1 \in \{-1, 1\}$ and  let $\Z$ be the $n \times 1$ vector of random variables $Z_1, ..., Z_n$ and $\z$ be the value of $\Z$. Let $\X_W$, $\T_W$ and $\R_W$ denote the matrices $\X$, $\T$ and $\R$ where each row $i$ corresponding to data point $i$ is multiplied by $W_i$. Conditioning on $\X = \x$, let $w_i  = \frac{p_T(x_i)}{p_S(x_i)} $ and $\x_w$, $\T_w$ and $\R_w$ denote the matrices $\x$, $\T$ and $\R$ where each row corresponding to data point $i$ is multiplied by $w_i$.

When $n_1 = n_0 = n/2$, the difference between the means of the weighted covariates of the treatment and control group can be written as:
\begin{align*}
\frac{2}{n}\sum_{Z_i = 1} w_i x_i - \frac{2}{n}\sum_{Z_i = -1} w_i x_i = \frac{2}{n}\x_w^T\Z.  
\end{align*}
In Definition~\ref{def:balance} we define a balance condition based on the Mahalanobis distance between $\frac{2}{n}\sum_{Z_i = 1} w_i x_i$ and  $\frac{2}{n}\sum_{Z_i = -1} w_i x_i $ calculated from $\x_w^T\Z$. 
The Mahalanobis distance of $\x_w\Z$ is
\begin{align*}
    M(\frac{2}{n} \x_w\Z) &= \frac{2}{n} \Z^T \x_w   [Cov(\frac{2}{n}\x_w^T \Z)]^{-1} \frac{2}{n}\x_w^T \Z \\
    &= \Z^T \x_w   [Cov(\x_w^T \Z)]^{-1} \x_w^T \Z.
\end{align*} \anup{Missing a factor of $2/n$.} \my{ we have $4/n^2$ outside of the Cov, and $n^2/4$ coming out from the cov? so they cancel out}
Let $V = Cov(\x_w^T \Z )^{-1/2} \x_w^T\Z$ so that $Cov(V) = \I$.  The Mahalanobis distance becomes 
\begin{align*}
   M(\frac{2}{n}\x_w\Z) &=  \norm{V}^2. 
\end{align*}
We now define Target Balance: \anup{Given that this is the central contribution of the paper, this definition should appear before the Analysis section.} 
\begin{definition}[Target Balance]

\label{def:balance}
Define the balance condition:
\begin{align*}
\phi =
    \begin{cases}
      1, & \text{if}\ M(\frac{2}{n}\x_w\Z) ) = \norm{V}^2 < a \\
      0, & \text{otherwise}
    \end{cases}
\end{align*}
\end{definition}

First we note that
\begin{align*}
    \phi(\x, \A) = \phi(\x, 1-\A),
\end{align*}
which satisfies the condition in  Theorem~\ref{thm:unbiased}. Therefore, conditioning on Target Balance, the importance-weighted estimator is an unbiased estimator of the target's ATE:
\begin{corollary}
\begin{align*}
     \mathbb{E}_S \left[\hat{\tau}^S_Y  |  \phi =1 \right] = \tau^T_Y.
\end{align*}
\end{corollary}


In order to calculate the distance $ M(\frac{2}{n} \x_w\Z)$ we need to calculate $Cov(\x_w^T\Z)$. We make use of the following result from Section 3.2 of \citep{harshaw2019balancing}]: when $n_0 = n_1 = n/2$, $Cov(\Z) = (n\mathbf{I} - \mathbf{1}\mathbf{1}^T)/(n-1)$ with $\mathbf{I}$ being the identity matrix and $\mathbf{1}$ a vector whose every entry is one. 
Then we can calculate $Cov(\x_w^T\Z)$ as follow:
\begin{align*}
    Cov(\x_w^T \Z) 
    &= \x_w^T \EE[  \Z \Z^T ] \x_w- \EE[\x_w^T \Z] \EE[\x_w^T \Z]^T\\
   % &= \x_w^T \EE[  \Z \Z^T ] \x_w -  \x_w^T \EE[ \Z] \EE[\x_w^T \Z]^T \\
    &= \frac{1}{n-1} \x_w^T (n\mathbf{I} - \mathbf{1}\mathbf{1}^T) \x_w\text{ because } \EE[ \Z] = \mathbf{0} .
\end{align*}



\input{variance_linear_final}
%\input{variance_linear}
\input{variance-nonlinear}
%\input{variance-nonlinear2}
%\input{variance-nonlinear3}
\input{optimality}



==> optimality.tex <==
\subsubsection{Optimality}
\label{sec:optimality}
Consider the first term $\gamma^T \EE[V V^T| \E ] \gamma$ in Lemma ~\ref{lem:variance_decomposition_normalized}. Since $\x_w^T\Z$ is asymptotically normal, $V$ is asymptotically a standard multivariate normal distribution.
We upper bound the first term:
\begin{align}
\label{eq:worst_case_bound}
    \gamma^T \EE[V V^T| \E ] \gamma \leq \|\gamma\|_2^2 \|\EE[V V^T| \E ]\|,
\end{align}
where equality holds when $\gamma$ is parallel to the eigenvector with the largest eigenvalue of $\EE[V V^T| \E ]$.
%Let $\e_1, ..., \e_m$ and $\lambda_1, .., \lambda_m$ be the eigenvectors and corresponding eigenvalues of a matrix $\M$. Following \citep{harshaw2019balancing}, we write $\gamma$ as a linear combination of $\e_1, .., \e_m$ and get:
%\begin{align*}
%   \gamma = \norm{\gamma}\sum_{i=1}^m \eta_i \e_i ,
%\end{align*}
%where $\eta_i = \langle \gamma, \e_i \rangle/\norm{\gamma}$. 
%Therefore, 
%\begin{align*}
%\label{eq:eigen_decomposition}
%   \gamma^T \M \gamma = \norm{\gamma}^2\sum_{i=1}^m \eta_i^2 \lambda_i.
%\end{align*}
We want to condition on event $\E$ with $P(\E) = 1- \alpha $ so as to minimize $\gamma^T \EE[V V^T| \E ] \gamma$. From Eq.~\ref{eq:worst_case_bound}, we want to pick $\E$ that minimize the largest eigenvalue of $\EE[V V^T| \E ]$. Now we will show that if $V$ satisfies some symmetry properties which the standard multivariate normal distribution satisfies, then given a rejection threshold $\alpha$, our balancing method achieves the greatest variance reduction. 
\begin{lemma}
\label{lem:optimality}
Let $W \in \mathcal{R}^d$ be a random variable with pdf $p(W)$ satisfying:
\begin{itemize}
    \item For any permutation $\pi$ that permutes the covariates, $p(w) = p(\pi(w))$
\item For any $u$ and $v$ such that $|u_i| = |v_i|~\forall 1 \le i \le d$, then $p(u) = p(v)$.
\end{itemize}
Let $\mathcal{S}_{\alpha}$ be the set of  events $\E$ such that $\PP(\E ) = 1- \alpha$. Let $\Phi_{\alpha}$ be the event: $ \norm{W} \le w_{\alpha}$ where $w_{\alpha}$ is defined such that $\PP(\norm{W} \le w_{\alpha}) = 1 - \alpha$. Let $\lambda(\M)$ denote the largest eigenvalue of matrix $\M$.
Then:
\begin{align*}
    \lambda( \EE[W W^T| \Phi_{\alpha} ] )  = \min_{\E \in \mathcal{S}_{\alpha}} \lambda( \EE[W W^T| \E ] )
\end{align*}
\end{lemma}
In other words, among all events with probability $1-\alpha$,  the largest eigenvalue of $\EE[W W^T | \E]$ is the smallest when $\E = \Phi_{\alpha}$. 

We now present the optimality of Target Balance. From Lemma~\ref{lem:optimality}, the largest eigenvalue of $\EE[VV^T | \E]$ in the first term of the decomposition in Lemma~\ref{lem:variance_decomposition_normalized} is the smallest when $\E$ is the event $\norm{V}^2 < v_{\alpha}$. Therefore, in the worst case when $\gamma$ is parallel to the eigenvector with the largest eigenvalue, the first term is the smallest when $\E$ is the event $\norm{V}^2 < v_{\alpha}$. 
\begin{theorem}
\label{thm:optimality}
Let $n_1 = n_0 = n/2$. Let $\mathcal{B}$ be the set of functions $\rho$ such that $\rho$ only depends on $\X$ and $\A$, $\rho(\X, \A) = \rho(\X, 1-\A)$  and $\PP(\rho = 1 | \x) = 1 - \alpha$. Let $\phi_{\alpha}$ be the balance condition in Definition~\ref{def:balance} with the threshold $a$ be such that $\PP(\phi_{\alpha} = 1| \x) = 1- \alpha$. Let $\norm{\beta}_{Cov(\x_w \Z)^{-1}}$ be the $Cov(\x_w \Z)^{-1}$-weighted norm \footnote{Given a vector $v \in \mathcal{R}^d$ and a matrix $M \in \mathcal{R}^{d \times d}$, the $M$-weighted norm of of $v$ is defined as $(v^T M v)^{1/2}$.} of $\beta$ and $L$ be any constant. Then %Then if $\x_w^T\Z$ is a multivariate normal\footnote{Due to the finite central limit theorem, $\x_w^T\Z$ is asymptotically normal.}:
\begin{align*}
 &\max_{\norm{\beta}_{Cov(\x_w \Z)^{-1}} \le L }   \text{as-var}_S(\hat{\tau}^S_Y | \x, \phi_{\alpha}=1) \\&= \min_{\rho \in \mathcal{B}} ~~ \max_{\norm{\beta}_{Cov(\x_w \Z)^{-1}} \le L }   \text{as-var}_S(\hat{\tau}^S_Y | \x, \rho = 1)
\end{align*}
%\my{ can this condition $\norm{\beta}_{Cov(\x_w \Z)^{-1}} \le L $ be converted to something more natural?}
\end{theorem}

Since the coefficient $\beta$ in the model is unknown, Theorem~\ref{thm:optimality} shows that for the worst case $\beta$, Target Balance achieves the minimum asymptotic variance among all symmetric balance conditions with the same rejection probability. 

\if0
\subsection{Previous attempt}
% \begin{align*}
% |U| \le \norm{\beta} \norm{V}\\
% |U| \le \norm{\gamma} \norm{W}
% \end{align*}
% In the worst case $|U| = \norm{\beta} \norm{V}$ So $U < u $ is equal to $\norm{V} < v$. 
Let $V = \x_w^T \Z$ and $W = Cov(V)^{-1/2} V $. Then $Cov(W) = \I$, $U = \beta^T V$. Let $\E$ be an event such that:
\begin{align*}
    &\EE[W_i | \E ] =0 \\
    &\EE[W_i  | \E, W_j] = 0 \\
    &\EE[W_i^2 | \E ] = \EE[W_j^2|\E] ~\forall i, j
\end{align*}
%and  the balance condition we defined above is:
\begin{align*}
    Cov(\beta^T \x^T \Z | \E) = \beta^T Cov(\x^T \Z | \E) \beta = \beta^T Cov(V | \E) \beta
\end{align*}
\begin{align*}
  Var(U| \E) = & Var(\beta^T V | \E)  \\
    = & Var(\beta^T  Cov(V)^{1/2}  Cov(V)^{-1/2} V |\E)   
    \\ = &  Var(\gamma^T W|\E) \text{ where }  \gamma^T =  \beta^T  Cov(V)^{1/2} 
    \\ = & Var(\sum_{i=1}^d \gamma_i W_i | \E ) 
    \end{align*}
    We have:
    \begin{align*}
        Cov(W_i, W_j | \E) &= \EE[W_i W_j | \E] \text{ because $\EE[W_i | \E ] =0$}\\
        &= \EE[  \EE[W_i W_j | \E, W_j] | \E] \\
        &= \EE[ W_j \EE[W_i  | \E, W_j] | \E] \\
        &= \EE[W_j \cdot 0 ] \text{ because $\EE[W_i  | \E, W_j] = 0$} \\
        &= 0
    \end{align*}
    Then:
    \begin{align*}
    &Var(\sum_{i=1}^d \gamma_i W_i | \E ) \\
     = & \sum_{i=1}^d \gamma_i^2 \EE(W_i^2 | \E) \text{ because $Cov(W_i, W_j |\E ) = 0$ and $\EE[W_i | \E] = 0$} \\
      = & \sum_{i=1}^d \gamma_i^2 \EE( \sum_{j=1}^d \frac{W_j^2}{d} \bigg| \E) \text{ because $\EE[W_i^2 | \E ] = \EE[W_j^2|\E]$} \\
      &= (\sum_{i=1}^d \gamma_i^2) \EE( W^TW| \E)
\end{align*}
The distance condition is equal to $W^T W < a$
% When $\gamma$ and $W$ are linearly dependent \my{ show that the equality $|U| =  \norm{\gamma} \norm{W}$ can happen, otherwise we can also just write $|U| \le \norm{\beta} \norm{V} $ but if the equality can't happen then it's not tight }, then $|U| = \norm{\gamma} \norm{W}$, therefore $|U| < u_{\alpha}$ is equivalent to:
% \begin{align*}
%     \norm{W} = W^T W < \frac{u_{\alpha}}{\norm{\gamma}}
% \end{align*}
% % \my{ refine this } 
\fi

==> variance-nonlinear.tex <==
\subsection{Variance for non linear model}
We assume that $n_1 = n_0 = n/2$. 
First we add a bias term $1$ to the end of $x_1, .., x_n$ so that $x_i$ has dimension $d+1$. 
Define 
\begin{align}
    T_i &= \frac{Y_i^1 + Y_i^0}{2}
\end{align}

Conditioning on $\X = \x, \Y = \y$, we can do linear regression on $\T$ and $\x$ and obtain: 
\begin{align}
    \ttt  = \beta^T \x  + \rr 
\end{align}
where $\rr$ is orthogonal to the span of $\x$. 

% Let $ \frac{p_T(X)}{p_S(X)}X = \frac{p_T(X)}{p_S(X)} X$.
% \begin{align}
%  %   \EE_S(Z) &= \EE_S \left(\frac{p_T(X)}{p_S(X)} \epsilon \right) = \EE_T( \epsilon) = 0 \\
%     \EE_S(\frac{p_T(X)}{p_S(X)}X) &= \EE_S \left(\frac{p_T(X)}{p_S(X)} X\right) = \EE_T(X)  
% \end{align}

% \begin{align}
%     Cov_S(\frac{p_T(X)}{p_S(X)}X) = Cov_S\left(\frac{p_T(X)}{p_S(X)} X \right) 
%     &= \EE_S \left(\frac{p_T(X)}{p_S(X)}   \right) ^2 XX^T - \left( \EE_S \frac{p_T(X)}{p_S(X)} X \right) \left( \EE_S \frac{p_T(X)}{p_S(X)} X \right)^T \\
%     &= \EE_T \left [\frac{p_T(X)}{p_S(X)} XX^T \right ] - (\EE_T X)(\EE_T X)^T
% \end{align}

Let $Z_i = 2A_i - 1 \in \{-1, 1\}$. Let $\x_w$, $\ttt_w$ and $\rr_w$ denote the matrices $\x$, $\ttt$ and $\rr$ where each row corresponding to data point $i$ is multiplied by $w_i$.
Let 
\begin{align}
\varphi(\x, \A) =  \x_w^T \Z [Cov(\x_w^T \Z)]^{-1} \Z^T \x_w < a
\end{align}
be the balancing condition where
\begin{align}
    Cov(\x_w^T \Z) 
    &= \EE[ \x_w^T \Z \Z^T \x_w] - \EE[\x_w^T \Z] \EE[\x_w^T \Z]^T\\
    &= \x_w^T  \EE[ \Z \Z^T]\x_w -  \x_w^T \EE[ \Z] \EE[\x_w^T \Z]^T \\
    &=   \x_w^T  \EE[ \Z \Z^T]\x_w \text{ because } \EE[ \Z] = \mathbf{0}
\end{align}
where since $\Z$ is the randomization design that make $n_0 = n_1$ we have $\EE[\Z \Z^T] = Cov(\Z) = (n\mathbf{I} - \mathbf{1}\mathbf{1}^T)/(n-1)$ with $\mathbf{I}$ being the identity matrix and $\mathbf{1}$ is a $d+1$-dimensional vector of $1$ (Section 3.2, page 8, \citep{harshaw2019balancing}). 

Therefore $\varphi(\x, \A)$ can be calculated by:
\begin{align}
\varphi(\x, \A) =  \frac{1}{n-1} \x_w^T \Z [\x_w^T  (n\mathbf{I} - \mathbf{1}\mathbf{1}^T) \x_w]^{-1} \Z^T \x_w < a
\end{align}


First we note that
\begin{align}
    \varphi(\X, \A) = \varphi(\X, 1-\A)
\end{align}
which satisfies the condition in Lemma~\ref{lem:helper}. Let $\phi(\X, \Z)$ denote $\varphi(\X, \A)$


% \begin{align}
%      \var_S(Z) = \var_S\left(\frac{p_T(X)}{p_S(X)} \epsilon \right) 
%     &= \EE_S \left(\frac{p_T(X)}{p_S(X)} \epsilon \right) ^2  - \left( \EE_S \frac{p_T(X)}{p_S(X)} \epsilon \right) ^2 \\
%     &= \EE_T \left [\frac{p_T(X)}{p_S(X)} ({\epsilon})^2\right ] - (\EE_T \epsilon^0)^2 \\
%     &= \EE_T \left [\frac{p_T(X)}{p_S(X)} ({\epsilon})^2\right ] \text{ because } \EE_T \epsilon = 0\\
%     &= \EE_T \left [\frac{p_T(X)}{p_S(X)} \right] \EE[ {\epsilon}^2 ] \text{because  $\frac{p_T(X)}{p_S(X)}$ and $\epsilon$ are independent} \\
%     &= \EE_T \left [\frac{p_T(X)}{p_S(X)} \right] \text{ because } \EE[ \epsilon^2 ]=1
% \end{align}
% \begin{align}
%     cov_S(\frac{p_T(X)}{p_S(X)}X,R) &= \EE_S[\frac{p_T(X)}{p_S(X)}XR] - \EE_S[\frac{p_T(X)}{p_S(X)}X] \EE_S[R] \\
%     &= \EE_S\left[ \frac{p_T(X)^2}{p_S(X)^2} X \epsilon^0\right] - 0 
% \end{align}


First we analyze the variance of $\hat{\tau}$ without the balance condition.
\begin{lemma}
Assume $n_0=n_1 = n/2$
\begin{align}
    \var_S(\hat{\tau}^S_Y | \x, \y) = \beta^T Cov(\x_w^T \Z)  \beta +  Cov(\rr_w^T\Z) 
\end{align}
\end{lemma}
\begin{proof}
We have 
\begin{align}
    \EE[\hat{\tau}^S_Y | \x, \y]
    &= \frac{2}{n} ( \sum_{i=1}^n w_i \EE[A_i  ] y^1_i -  \sum_{i=1}^n w_i (1-A_i ) y^0_i ) \\
    &= \frac{1}{n}\sum_{i=1}^n w_i (y^1_i - y^0_i) \text{ because $\EE[A_i  ] = 1/2$ }
\end{align}

Then using Lemma 1 in \cite{harshaw2019balancing}: 
\begin{align}
    &\frac{n^2}{4}\var_S(\hat{\tau}^S_Y | \x, \y) \\
    &= \frac{n^2}{4} \EE \left[(\hat{\tau}^S_Y - \mathbb{E}[\hat{\tau}^S_Y | \x, \y] )^2 | \x,\y \right] \\
    &=  \ttt_w^T Cov(\Z) \ttt_w \text{ by Lemma 1 in \cite{harshaw2019balancing}}\\
    &=  \beta^T \x_w^T Cov(\Z) \x_w \beta + \rr_w^T Cov(\Z) \rr_w + 2 \beta^T \x_w^T Cov(\Z) \rr_w \text{ using the decomposition in \cite{harshaw2019balancing}} \\
    &=  \beta^T Cov(\x_w^T \Z)  \beta +  Cov(\rr_w^T\Z)  + 2 \beta^T \x_w^T Cov(\Z) \rr_w 
\end{align}

The last term:
\begin{align}
    &\x_w^T Cov(\Z) \rr_w \\
    &= \x_w^T (n\I - \1 \1^T) \rr_w = n \x_w^T \rr_w - (\x_w^T \1)(\1^T \rr_w) \\
    &= 0 \text{ because $\rr_w$ is orthogonal to $\x_w$ and $\rr_w$ is orthogonal to $\1$}
    % &= \beta^T \x_w^T \EE[\Z \Z^T] \rr_w \text{ because $\EE[\Z] = \mathbf{0}$}\\
      %&= \EE[ \Z^T \rr_w  \x_w^T \Z] \text{ because $\Z^T \rr_w$ and  $\x_w^T \Z$ are 1D vector so they can swap order}\\
    %   &= \EE[ \Z^T  \R_w  \X_w^T \Z] = \EE \sum_i \X_w(i) \R_w(i) = n \EE X_w (T_w - \beta_A X_w) =0\\
    %  &= \EE[ \Z^T \mathbf{0} \Z] \text{ because $\rr_w$ and $ \x_w $ are orthogonal}\\
    %  &= 0
\end{align}
%\anup{$\rr_w  \x_w^T \neq 0$ as it is a matrix. But the final claim still holds as the sum of diagonal elements of $\rr_w  \x_w^T$ is $0.$}
\end{proof}

Now we analyze the variance of $\hat{\tau}$ with the balance condition:
\begin{lemma}
Suppose $n_1 = n_0 = n/2$ and using the balance condition

\begin{align}
\varphi(\x, \A) = \phi(\x, \Z) =  \x_w^T \Z [cov(\x_w^T \Z)]^{-1} \Z^T  \x_w  =  \frac{1}{n-1} \x_w^T \Z [\x_w^T  (n\mathbf{I} - \mathbf{1}\mathbf{1}^T) \x_w]^{-1} \Z^T \x_w < a
\end{align}
Suppose that $\x_w^T \Z$ and $\rr_w^T \Z$ has normal distribution (which is implied when $n$ is very large, using finite CLT \cite{li2016general}). Then: 
\begin{align}
    \var_S(\hat{\tau}^S_Y | \x, \y, \phi(\x, \Z)) =\frac{P(\chi^2_{k+2} \le a)}{P(\chi^2_k \le a)} \beta^T Cov(\x_w^T \Z) \beta + Cov(\rr_w^T \Z) 
\end{align}
\end{lemma}
\begin{proof}

First we will show that: 
\begin{align}
\EE \left[(\hat{\tau}^S_Y - \mathbb{E}[\hat{\tau}^S_Y | \x, \y] )^2 | \x,\y, \phi(\x, \Z) \right] 
    = \frac{4}{n^2} \ttt_w^T Cov(\Z | \phi(\x, \Z)) \ttt_w 
    \end{align}


We have 
\begin{align}
    \EE[\hat{\tau}^S_Y | \x, \y, \phi(\x, \Z)]
    &= \frac{2}{n} ( \sum_{i=1}^n w_i \EE[A_i | \phi(\x, \Z) ] y^1_i -  \sum_{i=1}^n w_i (1-A_i  | \phi(\x, \Z)) y^0_i ) \\
    &= \frac{1}{n}\sum_{i=1}^n w_i (y^1_i - y^0_i) \text{ because $\EE[A_i  | \phi(\x, \Z)] = 1/2$ from lemma~\ref{lem:helper}}
\end{align}

Then using Lemma A1 in \cite{harshaw2019balancing} we have: 
\begin{align}
    \hat{\tau}^S_Y - \mathbb{E}[\hat{\tau}^S_Y | \x, \y, \phi(\x, \Z)] = \frac{2}{n} <\Z, \ttt_w>
\end{align}
Then:
\begin{align}
& \EE \left[(\hat{\tau}^S_Y - \mathbb{E}[\hat{\tau}^S_Y | \x, \y] )^2 | \x,\y, \phi(\x, \Z) \right] \\
&= \frac{4}{n^2} \ttt_w^T \EE[\Z\Z^T | \x, \y, \phi(\x, \Z)] \ttt_w \\
&= \frac{4}{n^2} \ttt_w^T \EE[\Z\Z^T |  \phi(\x, \Z)] \ttt_w \\
    &= \frac{4}{n^2} \ttt_w^T Cov(\Z| \phi(\x, \Z)) \ttt_w \text{ because } \EE[\Z | \phi(\x, \Z) ] = 0 \text{ from Lemma~\ref{lem:helper}}
    \end{align}
Therefore: 
\begin{align}
    &\frac{n^2}{4}\var_S(\hat{\tau}^S_Y | \x, \y, \phi(\x, \Z) ) \\
    &= \frac{n^2}{4} \EE \left[(\hat{\tau}^S_Y - \mathbb{E}[\hat{\tau}^S_Y | \x, \y] )^2 | \x,\y, \phi(\x, \Z) \right] \\
    &= \ttt_w^T Cov(\Z | \phi(\x, \Z)) \ttt_w \\
    &=  \beta^T \x_w^T Cov(\Z| \phi(\x, \Z)) \x_w \beta + \rr_w^T Cov(\Z| \phi(\x, \Z)) \rr_w + 2 \beta^T \x_w^T Cov(\Z| \phi(\x, \Z)) \rr_w \\ &\text{ using the decomposition in \cite{harshaw2019balancing}} \\
    &=  \beta^T Cov(\x_w^T \Z| \phi(\x, \Z)) \beta + Cov(\rr_w^T \Z| \phi(\x, \Z))  + 2 \beta^T \x_w^T Cov(\Z| \phi(\x, \Z)) \rr_w
\end{align}


The first term $Cov(\x_w^T \Z)$ is the covariance of the truncated distribution of $\x_w^T \Z$. $\x_w^T \Z$ has a symmetric distribution and by finite population CLT \citep{li2016general}, when $n$ is large
$\frac{2}{n}\x_w^T \Z$ converges in distribution to a normal distribution. By theorem 3.1 from ~\cite{rubin2011causal}:
\begin{align}
    Cov( \x_w^T \Z |  \phi(\x, \Z) ) = \frac{P(\chi^2_{k+2} \le a)}{P(\chi^2_k \le a)} Cov(\x_w^T \Z) 
\end{align}
For $\X = \x$, $\T = \ttt$:
\begin{align}
\beta = (\x^T\x)^{-1}\x^T \ttt
\end{align}
by calculation. 
% Is 
% \begin{align}
% \beta = (\X^T\X)^{-1}\X^T \T
% \end{align}

% Where $\X$ is $n$ iid RVs $X_1, ..., X_n$  and $\T$ is $n$ iid RVs $T_1, .., T_n$? 
% $\beta = \arg \min_{\beta} \EE_S (y-\beta x)^2.$

For the second term, we will first show that $U = ( \x_w^T \Z, \rr_w^T \Z) = ( \x_w^T, \rr_w^T) \Z $ is multivariate normal when $n$ is large. By definition $\beta = (\x^T \x)^{-1} \x^T \ttt$ and
\begin{align}
    \rr = \y - \x \beta = \y - \x (\x^T \x)^{-1} \x^T \ttt
\end{align}
Define random variable $\R$ (recall that $\Y = (Y_1, ..., Y_n)$ and $\X = (X_1, ..., X_n)$ are random variables):
\begin{align}
    \R = \T - \X (\X^T \X)^{-1} \X^T \T
\end{align}
$\R = (R_1, .., R_n)$ where: 
\begin{align}
    R_i = T_i - X_i^T (\X^T \X)^{-1} \X^T \T
\end{align}
Let $V_i = \frac{p_T(X_i)}{p_S(X_i)}\begin{bmatrix}
           X_i \\
           R_i 
         \end{bmatrix}$ be the random variable created by stacking $\frac{p_T(X_i)}{p_S(X_i)}X_i$ and $\frac{p_T(X_i)}{p_S(X_i)}R_i$ together. 

Then let $i_1, .., i_{n/2}$ be randomly chosen from $1, ..,n$:
\begin{align}
    &S_n = \frac{V_{i_1} + ... V_{i_{n/2}}}{n/2} \\
    &= \frac{1}{n/2} \sum_{j \in \{i_1, .., i_{n/2}\}}  \frac{p_T(X_j)}{p_S(X_j)} \begin{bmatrix}
           X_j \\
           R_j 
         \end{bmatrix}
    \\
    &= \frac{1}{n/2} \sum_{j \in \{i_1, .., i_{n/2}\}} \frac{p_T(X_j)}{p_S(X_j)} \begin{bmatrix}
           X_j \\
           T_j - X_j^T (\X^T \X)^{-1} \X^T \T
         \end{bmatrix} 
\end{align}
\my{ we want to find the condition so that $S_n$ is asymtotically normal. We can't use CLT because $V_i's$ are identical but not idenpendent. I am afraid $S_n$ is asymtotically normal only when $(\X^T \X)^{-1} \X^T \T$ is a constant, i.e the model is linear}

 Since $ \x_w^T Cov(\Z) \rr_w = Cov( \rr_w^T \Z,  \x_w^T \Z ) = 0$, $\rr_w^T \Z$ and $\x_w^T \Z$ are uncorrelated. Since $(\rr_w^T \Z, \x_w^T \Z)$ is a multivariate normal and $\rr_w^T \Z$ and $\x_w^T \Z$ are uncorrelated,  $\rr_w^T \Z$ and $\x_w^T \Z$ are independent:
\begin{align}
    Cov(\rr_w^T \Z| \phi(\x, \Z)) = Cov(\rr_w^T \Z) 
\end{align}
The third term: 
\begin{align}
    &\beta^T\x_w^T Cov(\Z | \phi(\x, \Z) ) \rr_w \\
    &= \beta^T \x_w^T \EE[\Z \Z^T| \phi(\x, \Z)] \rr_w \text{ because $\EE[\Z| \phi(\x, \Z)] = \mathbf{0}$}\\
     &= \beta^T\EE[ \Z^T \rr_w \x_w^T \Z| \phi(\x, \Z)] \text{ because $\Z^T \rr_w$ and  $\x_w^T \Z$ are scalar so they can swap order} 
\end{align}
Therefore:
\begin{align}
    \var_S(\hat{\tau}^S_Y | \x, \y, \phi(\x, \Z)) =\frac{P(\chi^2_{k+2} \le a)}{P(\chi^2_k \le a)} \beta^T Cov(\x_w^T \Z) \beta + Cov(\rr_w^T \Z) 
\end{align}

\end{proof}

==> variance-nonlinear2.tex <==
\subsection{Variance for non linear model - Second attempt}
We assume that $n_1 = n_0 = n/2$. 
First we add a bias term $1$ to the end of $x_1, .., x_n$ so that $x_i$ has dimension $d+1$. 
Define 
\begin{align}
    T_i &= \frac{Y_i^1 + Y_i^0}{2}
\end{align}

Let $\beta = (\X^T \X)^{-1} \X^T \T$ and
\begin{align}
    \R = \T - \X (\X^T \X)^{-1} \X^T \T
\end{align}
We have $\R$ is orthogonal to $\X$ \my{is this true?} and: 
\begin{align}
    \T  = \beta^T \X  + \R
\end{align}


% Let $ \frac{p_T(X)}{p_S(X)}X = \frac{p_T(X)}{p_S(X)} X$.
% \begin{align}
%  %   \EE_S(Z) &= \EE_S \left(\frac{p_T(X)}{p_S(X)} \epsilon \right) = \EE_T( \epsilon) = 0 \\
%     \EE_S(\frac{p_T(X)}{p_S(X)}X) &= \EE_S \left(\frac{p_T(X)}{p_S(X)} X\right) = \EE_T(X)  
% \end{align}

% \begin{align}
%     Cov_S(\frac{p_T(X)}{p_S(X)}X) = Cov_S\left(\frac{p_T(X)}{p_S(X)} X \right) 
%     &= \EE_S \left(\frac{p_T(X)}{p_S(X)}   \right) ^2 XX^T - \left( \EE_S \frac{p_T(X)}{p_S(X)} X \right) \left( \EE_S \frac{p_T(X)}{p_S(X)} X \right)^T \\
%     &= \EE_T \left [\frac{p_T(X)}{p_S(X)} XX^T \right ] - (\EE_T X)(\EE_T X)^T
% \end{align}

Let $Z_i = 2A_i - 1 \in \{-1, 1\}$. Let $\x_W$, $\ttt_W$ and $\rr_W$ denote the matrices $\x$, $\ttt$ and $\rr$ where each row corresponding to data point $i$ is multiplied by $w_i$.
Let 
\begin{align}
\varphi(\x, \A) =  \x_W^T \Z [Cov(\x_W^T \Z)]^{-1} \Z^T \x_W < a
\end{align}
be the balancing condition where
\begin{align}
    Cov(\x_W^T \Z) 
    &= \EE[ \x_W^T \Z \Z^T \x_W] - \EE[\x_W^T \Z] \EE[\x_W^T \Z]^T\\
    &= \x_W^T  \EE[ \Z \Z^T]\x_W -  \x_W^T \EE[ \Z] \EE[\x_W^T \Z]^T \\
    &=   \x_W^T  \EE[ \Z \Z^T]\x_W \text{ because } \EE[ \Z] = \mathbf{0}
\end{align}
where since $\Z$ is the randomization design that make $n_0 = n_1$ we have $\EE[\Z \Z^T] = Cov(\Z) = (n\mathbf{I} - \mathbf{1}\mathbf{1}^T)/(n-1)$ with $\mathbf{I}$ being the identity matrix and $\mathbf{1}$ is a $d+1$-dimensional vector of $1$ (Section 3.2, page 8, \citep{harshaw2019balancing}). 

Therefore $\varphi(\x, \A)$ can be calculated by:
\begin{align}
\varphi(\x, \A) =  \frac{1}{n-1} \x_W^T \Z [\x_W^T  (n\mathbf{I} - \mathbf{1}\mathbf{1}^T) \x_W]^{-1} \Z^T \x_W < a
\end{align}


First we note that
\begin{align}
    \varphi(\X, \A) = \varphi(\X, 1-\A)
\end{align}
which satisfies the condition in Lemma~\ref{lem:helper}. Let $\phi(\X, \Z)$ denote $\varphi(\X, \A)$


% \begin{align}
%      \var_S(Z) = \var_S\left(\frac{p_T(X)}{p_S(X)} \epsilon \right) 
%     &= \EE_S \left(\frac{p_T(X)}{p_S(X)} \epsilon \right) ^2  - \left( \EE_S \frac{p_T(X)}{p_S(X)} \epsilon \right) ^2 \\
%     &= \EE_T \left [\frac{p_T(X)}{p_S(X)} ({\epsilon})^2\right ] - (\EE_T \epsilon^0)^2 \\
%     &= \EE_T \left [\frac{p_T(X)}{p_S(X)} ({\epsilon})^2\right ] \text{ because } \EE_T \epsilon = 0\\
%     &= \EE_T \left [\frac{p_T(X)}{p_S(X)} \right] \EE[ {\epsilon}^2 ] \text{because  $\frac{p_T(X)}{p_S(X)}$ and $\epsilon$ are independent} \\
%     &= \EE_T \left [\frac{p_T(X)}{p_S(X)} \right] \text{ because } \EE[ \epsilon^2 ]=1
% \end{align}
% \begin{align}
%     cov_S(\frac{p_T(X)}{p_S(X)}X,R) &= \EE_S[\frac{p_T(X)}{p_S(X)}XR] - \EE_S[\frac{p_T(X)}{p_S(X)}X] \EE_S[R] \\
%     &= \EE_S\left[ \frac{p_T(X)^2}{p_S(X)^2} X \epsilon^0\right] - 0 
% \end{align}


First we analyze the variance of $\hat{\tau}$ without the balance condition.
\begin{lemma}
Assume $n_0=n_1 = n/2$
\begin{align}
    \var_S(\hat{\tau}^S_Y) =  Cov(\beta^T\X_W^T \Z)   +  Cov(\R_W^T\Z) 
\end{align}
\end{lemma}
\begin{proof}
We have 
\begin{align}
    \EE[\hat{\tau}^S_Y ]
    &= \frac{2}{n} ( \sum_{i=1}^n  \EE[W_i A_i   Y^1_i] -  \sum_{i=1}^n \EE[W_i (1-A_i ) Y^0_i] ) \\
    &= \frac{2}{n} ( \sum_{i=1}^n \EE[A_i] \EE[W_i  Y^1_i] -  \sum_{i=1}^n \EE[1-A_i] \EE[W_i  Y^0_i] ) \\
    &= \frac{1}{n}\sum_{i=1}^n W_i (Y^1_i - Y^0_i) \text{ because $\EE[A_i  ] = 1/2$ }
\end{align}

Then using Lemma 1 in \cite{harshaw2019balancing}: 
\begin{align}
    &\frac{n^2}{4}\var_S(\hat{\tau}^S_Y ) \\
    &= \frac{n^2}{4} \EE \left[(\hat{\tau}^S_Y - \mathbb{E}[\hat{\tau}^S_Y ] )^2 |  \right] \\
    &=   Cov(\T_W^T\Z)  \text{ by Lemma 1 in \cite{harshaw2019balancing}}\\
    &=  Cov(\beta^T \X_W^T\Z)  + Cov(\R_W^T \Z)  + 2 Cov(\beta^T \X_W^T\Z, \R_W^T \Z)  \text{ using the decomposition in \cite{harshaw2019balancing}} 
\end{align}

The last term:
\begin{align}
    &Cov(\beta^T \X_W^T\Z, \R_W^T \Z) \\
    &= \EE[\beta^T \X_W^T \Z \Z^T \R_W]\text{ because $\EE[\Z] = \mathbf{0}$}\\
     &= \EE[ \Z^T \R_W  \beta^T \X_W^T \Z] \text{ because $\Z^T \R_W$ and  $\beta^T \X_W^T \Z$ are 1D vector so they can swap order}\\
     &= 0 \text{ because $\R_W$ and $ \beta \X_W $ are orthogonal}\\
\end{align}
\my{ more explanation why it's 0}
\anup{$\rr_W  \x_W^T \neq 0$ as it is a matrix. But the final claim still holds as the sum of diagonal elements of $\rr_W  \x_W^T$ is $0.$}
\end{proof}

Now we analyze the variance of $\hat{\tau}$ with the balance condition:
\begin{lemma}
Suppose $n_1 = n_0 = n/2$ and using the balance condition

\begin{align}
\varphi(\X, \A) = \phi(\X, \Z) =  \X_W^T \Z [cov(\X_W^T \Z)]^{-1} \Z^T  \X_W  =  \frac{1}{n-1} \X_W^T \Z [\X_W^T  (n\mathbf{I} - \mathbf{1}\mathbf{1}^T) \X_W]^{-1} \Z^T \X_W < a
\end{align}
Suppose that $\x_W^T \Z$ and $\rr_W^T \Z$ has normal distribution (which is implied when $n$ is very large, using finite CLT \cite{li2016general}). Then: 
\begin{align}
    \var_S(\hat{\tau}^S_Y | \phi(\x, \Z)) =\frac{P(\chi^2_{k+2} \le a)}{P(\chi^2_k \le a)} \beta^T Cov(\X_W^T \Z) \beta + Cov(\R_W^T \Z) 
\end{align}
\end{lemma}
\begin{proof}

First we will show that: 
\begin{align}
\EE \left[(\hat{\tau}^S_Y - \mathbb{E}[\hat{\tau}^S_Y ] )^2 | \phi(\x, \Z) \right] 
    = \frac{4}{n^2}  Cov(\T_W^T\Z | \phi(\x, \Z))  
    \end{align}


We have 
\begin{align}
    \EE[\hat{\tau}^S_Y |  \phi(\X, \Z)]
    &= \frac{2}{n} ( \sum_{i=1}^n  \EE[A_i | \phi(\X, \Z) ] \EE[W_i Y^1_i  | \phi(\X, \Z)]-  \sum_{i=1}^n \EE[1-A_i  | \phi(\X, \Z)] \EE[Y^0_i W_i || \phi(\X, \Z)] ) \\&\text{ because $A_i$ and $W_i Y^1_i$ are independent conditioned on $\phi(\X, \Z)$}\\
    &= \frac{1}{n}\sum_{i=1}^n \EE[W_i (Y^1_i - Y^0_i) | \phi(\X, \Z)] \text{ because $\EE[A_i  | \phi(\X, \Z)] = 1/2$ from lemma~\ref{lem:helper}}
\end{align}

Then using Lemma A1 in \cite{harshaw2019balancing} we have: \my{ need to double check}
\begin{align}
    \hat{\tau}^S_Y - \mathbb{E}[\hat{\tau}^S_Y |  \phi(\X, \Z)] = \frac{2}{n} \EE[ <\Z, \T_W> | \phi(\X, \Z)]
\end{align}
Then:
\begin{align}
& \EE \left[(\hat{\tau}^S_Y - \mathbb{E}[\hat{\tau}^S_Y ] )^2 | \phi(\X, \Z) \right] \\
&= \frac{4}{n^2} \EE[\T_W^T \Z\Z^T \T_W| \phi(\X, \Z)]  \\
    &= \frac{4}{n^2}  Cov(\T_W^T \Z| \phi(\X, \Z)) \T_W \text{ because } \EE[\Z | \phi(\X, \Z) ] = 0 \text{ from Lemma~\ref{lem:helper}}
    \end{align}
Therefore: 
\begin{align}
    &\frac{n^2}{4}\var_S(\hat{\tau}^S_Y |  \phi(\x, \Z) ) \\
    &= \frac{n^2}{4} \EE \left[(\hat{\tau}^S_Y - \mathbb{E}[\hat{\tau}^S_Y | ] )^2 |  \phi(\x, \Z) \right] \\
    &=  Cov(\T_W^T\Z | \phi(\X, \Z)) \T_W \\
    &=   Cov(\beta^T \X_W^T\Z| \phi(\X, \Z))  +  Cov(\R_W^T\Z| \phi(\X, \Z))  + 2  Cov(\beta^T \X_W^T\Z, \R_W^T\Z| \phi(\X, \Z)) \\ &\text{ using the decomposition in \cite{harshaw2019balancing}} 
\end{align}


The first term is the covariance of the truncated distribution of $\X_W^T \Z$. $\X_W^T \Z$. Since $X_i$'s are iid normal and \my{ some other conditions}, $X_i W_i$'s are iid normal and therefore $X_W^T \Z$ is normal. By theorem 3.1 from ~\cite{rubin2011causal}:
\begin{align}
    Cov( \X_W^T \Z |  \phi(\X, \Z) ) = \frac{P(\chi^2_{k+2} \le a)}{P(\chi^2_k \le a)} Cov(\X_W^T \Z) 
\end{align}
For the second term, we will first show that $U = ( \X_W^T \Z, \R_W^T \Z) = ( \X_W^T, \R_W^T) \Z $ is multivariate normal. \my{TODO}
 Since $ Cov( \R_W^T \Z,  \beta^T \x_W^T \Z ) = 0$, $\rr_W^T \Z$ and $\x_W^T \Z$ are uncorrelated. Since $(\rr_W^T \Z, \x_W^T \Z)$ is a multivariate normal and $\rr_W^T \Z$ and $\x_W^T \Z$ are uncorrelated,  $\rr_W^T \Z$ and $\x_W^T \Z$ are independent:
\begin{align}
    Cov(\rr_W^T \Z| \phi(\x, \Z)) = Cov(\rr_W^T \Z) 
\end{align}
The third term: 
\begin{align}
    &\beta^T\x_W^T Cov(\Z | \phi(\x, \Z) ) \rr_W \\
    &= \beta^T \x_W^T \EE[\Z \Z^T| \phi(\x, \Z)] \rr_W \text{ because $\EE[\Z| \phi(\x, \Z)] = \mathbf{0}$}\\
     &= \EE[ \Z^T \rr_W \beta^T\x_W^T \Z| \phi(\x, \Z)] \text{ because $\Z^T \rr_W$ and  $\beta^T\x_W^T \Z$ are scalar so they can swap order}\\
     &= \EE[ \Z^T \mathbf{0} \Z| \phi(\x, \Z)] \text{ because $\rr_W$ and $\x_W \beta$ are orthogonal}\\
     &= 0
\end{align}
Therefore:
\begin{align}
    \var_S(\hat{\tau}^S_Y | \x, \y, \phi(\x, \Z)) =\frac{P(\chi^2_{k+2} \le a)}{P(\chi^2_k \le a)} \beta^T Cov(\x_W^T \Z) \beta + Cov(\rr_W^T \Z) 
\end{align}

\end{proof}

==> variance-nonlinear3.tex <==
\subsection{Variance for non linear model - Third attempt}
We assume that $n_1 = n_0 = n/2$. 
First we add a bias term $1$ to the end of $x_1, .., x_n$ so that $x_i$ has dimension $d+1$. 
Define 
\begin{align}
    T_i &= \frac{Y_i^1 + Y_i^0}{2}
\end{align}

Let $\beta = \min \EE(T - \beta^T X)^2$ and 
\begin{align}
    R = T - \beta^T X
\end{align}
Then:
\begin{align}
 &\beta^T = \EE[YX^T] (\EE[XX^T])^{-1} \\
 &\EE[ R X^T ] = \mathbf{0} \text{ so } \EE[R] = 0 \text{ because the first dimension of $X$ is $1$}
\end{align}
% Let $\beta = (\X^T \X)^{-1} \X^T \T$ and
% \begin{align}
%     \R = \T - \X (\X^T \X)^{-1} \X^T \T
% \end{align}
% We have $\R$ is orthogonal to $\X$ \my{is this true?} and: 
% \begin{align}
%     \T  = \beta^T \X  + \R
% \end{align}


% Let $ \frac{p_T(X)}{p_S(X)}X = \frac{p_T(X)}{p_S(X)} X$.
% \begin{align}
%  %   \EE_S(Z) &= \EE_S \left(\frac{p_T(X)}{p_S(X)} \epsilon \right) = \EE_T( \epsilon) = 0 \\
%     \EE_S(\frac{p_T(X)}{p_S(X)}X) &= \EE_S \left(\frac{p_T(X)}{p_S(X)} X\right) = \EE_T(X)  
% \end{align}

% \begin{align}
%     Cov_S(\frac{p_T(X)}{p_S(X)}X) = Cov_S\left(\frac{p_T(X)}{p_S(X)} X \right) 
%     &= \EE_S \left(\frac{p_T(X)}{p_S(X)}   \right) ^2 XX^T - \left( \EE_S \frac{p_T(X)}{p_S(X)} X \right) \left( \EE_S \frac{p_T(X)}{p_S(X)} X \right)^T \\
%     &= \EE_T \left [\frac{p_T(X)}{p_S(X)} XX^T \right ] - (\EE_T X)(\EE_T X)^T
% \end{align}

Let $Z_i = 2A_i - 1 \in \{-1, 1\}$. Let $\x_W$, $\ttt_W$ and $\rr_W$ denote the matrices $\x$, $\ttt$ and $\rr$ where each row corresponding to data point $i$ is multiplied by $w_i$.
Let 
\begin{align}
\varphi(\x, \A) =  \x_W^T \Z [Cov(\x_W^T \Z)]^{-1} \Z^T \x_W < a
\end{align}
be the balancing condition where
\begin{align}
    Cov(\x_W^T \Z) 
    &= \EE[ \x_W^T \Z \Z^T \x_W] - \EE[\x_W^T \Z] \EE[\x_W^T \Z]^T\\
    &= \x_W^T  \EE[ \Z \Z^T]\x_W -  \x_W^T \EE[ \Z] \EE[\x_W^T \Z]^T \\
    &=   \x_W^T  \EE[ \Z \Z^T]\x_W \text{ because } \EE[ \Z] = \mathbf{0}
\end{align}
where since $\Z$ is the randomization design that make $n_0 = n_1$ we have $\EE[\Z \Z^T] = Cov(\Z) = (n\mathbf{I} - \mathbf{1}\mathbf{1}^T)/(n-1)$ with $\mathbf{I}$ being the identity matrix and $\mathbf{1}$ is a $d+1$-dimensional vector of $1$ (Section 3.2, page 8, \citep{harshaw2019balancing}). 

Therefore $\varphi(\x, \A)$ can be calculated by:
\begin{align}
\varphi(\x, \A) =  \frac{1}{n-1} \x_W^T \Z [\x_W^T  (n\mathbf{I} - \mathbf{1}\mathbf{1}^T) \x_W]^{-1} \Z^T \x_W < a
\end{align}


First we note that
\begin{align}
    \varphi(\X, \A) = \varphi(\X, 1-\A)
\end{align}
which satisfies the condition in Lemma~\ref{lem:helper}. Let $\phi(\X, \Z)$ denote $\varphi(\X, \A)$


% \begin{align}
%      \var_S(Z) = \var_S\left(\frac{p_T(X)}{p_S(X)} \epsilon \right) 
%     &= \EE_S \left(\frac{p_T(X)}{p_S(X)} \epsilon \right) ^2  - \left( \EE_S \frac{p_T(X)}{p_S(X)} \epsilon \right) ^2 \\
%     &= \EE_T \left [\frac{p_T(X)}{p_S(X)} ({\epsilon})^2\right ] - (\EE_T \epsilon^0)^2 \\
%     &= \EE_T \left [\frac{p_T(X)}{p_S(X)} ({\epsilon})^2\right ] \text{ because } \EE_T \epsilon = 0\\
%     &= \EE_T \left [\frac{p_T(X)}{p_S(X)} \right] \EE[ {\epsilon}^2 ] \text{because  $\frac{p_T(X)}{p_S(X)}$ and $\epsilon$ are independent} \\
%     &= \EE_T \left [\frac{p_T(X)}{p_S(X)} \right] \text{ because } \EE[ \epsilon^2 ]=1
% \end{align}
% \begin{align}
%     cov_S(\frac{p_T(X)}{p_S(X)}X,R) &= \EE_S[\frac{p_T(X)}{p_S(X)}XR] - \EE_S[\frac{p_T(X)}{p_S(X)}X] \EE_S[R] \\
%     &= \EE_S\left[ \frac{p_T(X)^2}{p_S(X)^2} X \epsilon^0\right] - 0 
% \end{align}


First we analyze the variance of $\hat{\tau}$ without the balance condition.
\begin{lemma}
Assume $n_0=n_1 = n/2$
\begin{align}
    \var_S(\hat{\tau}^S_Y) =  Cov(\beta^T\X_W^T \Z)   +  Cov(\R_W^T\Z) 
\end{align}
\end{lemma}
\begin{proof}
We have 
\begin{align}
    \EE[\hat{\tau}^S_Y ]
    &= \frac{2}{n} ( \sum_{i=1}^n  \EE[W_i A_i   Y^1_i] -  \sum_{i=1}^n \EE[W_i (1-A_i ) Y^0_i] ) \\
    &= \frac{2}{n} ( \sum_{i=1}^n \EE[A_i] \EE[W_i  Y^1_i] -  \sum_{i=1}^n \EE[1-A_i] \EE[W_i  Y^0_i] ) \\
    &= \frac{1}{n}\sum_{i=1}^n W_i (Y^1_i - Y^0_i) \text{ because $\EE[A_i  ] = 1/2$ }
\end{align}

Then using Lemma 1 in \cite{harshaw2019balancing}: 
\begin{align}
    &\frac{n^2}{4}\var_S(\hat{\tau}^S_Y ) \\
    &= \frac{n^2}{4} \EE \left[(\hat{\tau}^S_Y - \mathbb{E}[\hat{\tau}^S_Y ] )^2 |  \right] \\
    &=   Cov(\T_W^T\Z)  \text{ by Lemma 1 in \cite{harshaw2019balancing}}\\
    &=  Cov(\beta^T \X_W^T\Z)  + Cov(\R_W^T \Z)  + 2 Cov(\beta^T \X_W^T\Z, \R_W^T \Z)  \text{ using the decomposition in \cite{harshaw2019balancing}} 
\end{align}

The last term:
\begin{align}
    &Cov(\beta^T \X_W^T\Z, \R_W^T \Z) \\
    &= \EE[ \beta^T \X_W^T \Z \Z^T \R_W] - \EE[\beta^T \X_W^T \Z] \EE[ \Z^T \R_W] \\
     &=  \EE[ \beta^T\X_W^T \Z \Z^T \R_W] - \EE[ \beta^T \X_W^T \Z] \EE[ \Z^T] \EE[ \R_W] \text{ because $\Z$ and $\R_W$ are independent}\\
     &= \EE[ \beta^T \X_W^T \Z \Z^T \R_W]  \text{ because $\EE[\Z] = \mathbf{0}$}\\
     &=\sum_i \sum_j \EE[\alpha_i Z_i Z_j R_j] \text{where $\alpha^T = \beta^T \X_W^T$} \\
     &= \sum_i \EE[\alpha_i 1 R_i] + \sum_{i \neq j} \EE[\alpha_i Z_i Z_j] \EE[R_j] \text{ because $Z_i^2 = 1$ and $R_j$ is independent of $X_i$ and $Z_i, Z_j$ when $i \neq j$} \\
     &=0 \text{ because $\EE[X_i R_i] = 0$ and $\EE[R_i] =0$}
\end{align}
\end{proof}
\begin{lemma}
\label{lem:assumption}
If $\X_W\Z$ and $(\X_W\Z, \R_W\Z)$ has a multivariate normal distribution then $R$ is independent of $X$. 
\end{lemma}
\begin{proof}
\my{TODO}
\end{proof}
Now we analyze the variance of $\hat{\tau}$ with the balance condition:
\begin{lemma}
Suppose $n_1 = n_0 = n/2$ and using the balance condition

\begin{align}
\varphi(\X, \A) = \phi(\X, \Z) =  \X_W^T \Z [cov(\X_W^T \Z)]^{-1} \Z^T  \X_W  =  \frac{1}{n-1} \X_W^T \Z [\X_W^T  (n\mathbf{I} - \mathbf{1}\mathbf{1}^T) \X_W]^{-1} \Z^T \X_W < a
\end{align}
Suppose that $\X_W^T \Z$ and $(\X_w^T, \R_W^T) \Z$ has normal distribution (which is true when $p_S(X)$ and $p_S(Y)$ are normal from Lemma~\ref{lem:assumption}, or when $n$ is very large, using finite CLT \cite{li2016general}). Then: 
\begin{align}
    \var_S(\hat{\tau}^S_Y | \phi(\x, \Z)) =\frac{P(\chi^2_{k+2} \le a)}{P(\chi^2_k \le a)} \beta^T Cov(\X_W^T \Z) \beta + Cov(\R_W^T \Z) 
\end{align}
\end{lemma}
\begin{proof}

First we will show that: 
\begin{align}
\EE \left[(\hat{\tau}^S_Y - \mathbb{E}[\hat{\tau}^S_Y ] )^2 | \phi(\x, \Z) \right] 
    = \frac{4}{n^2}  Cov(\T_W^T\Z | \phi(\x, \Z))  
    \end{align}


We have 
\begin{align}
    \EE[\hat{\tau}^S_Y |  \phi(\X, \Z)]
    &= \frac{2}{n} ( \sum_{i=1}^n  \EE[A_i | \phi(\X, \Z) ] \EE[W_i Y^1_i  | \phi(\X, \Z)]-  \sum_{i=1}^n \EE[1-A_i  | \phi(\X, \Z)] \EE[Y^0_i W_i || \phi(\X, \Z)] ) \\&\text{ because $A_i$ and $W_i Y^1_i$ are independent conditioned on $\phi(\X, \Z)$}\\
    &= \frac{1}{n}\sum_{i=1}^n \EE[W_i (Y^1_i - Y^0_i) | \phi(\X, \Z)] \text{ because $\EE[A_i  | \phi(\X, \Z)] = 1/2$ from lemma~\ref{lem:helper}}
\end{align}

Then using Lemma A1 in \cite{harshaw2019balancing} we have: \my{ need to double check}
\begin{align}
    \hat{\tau}^S_Y - \mathbb{E}[\hat{\tau}^S_Y |  \phi(\X, \Z)] = \frac{2}{n} \EE[ <\Z, \T_W> | \phi(\X, \Z)]
\end{align}
Then:
\begin{align}
& \EE \left[(\hat{\tau}^S_Y - \mathbb{E}[\hat{\tau}^S_Y ] )^2 | \phi(\X, \Z) \right] \\
&= \frac{4}{n^2} \EE[\T_W^T \Z\Z^T \T_W| \phi(\X, \Z)]  \\
    &= \frac{4}{n^2}  Cov(\T_W^T \Z| \phi(\X, \Z)) \T_W \text{ because } \EE[\Z | \phi(\X, \Z) ] = 0 \text{ from Lemma~\ref{lem:helper}}
    \end{align}
Therefore: 
\begin{align}
    &\frac{n^2}{4}\var_S(\hat{\tau}^S_Y |  \phi(\x, \Z) ) \\
    &= \frac{n^2}{4} \EE \left[(\hat{\tau}^S_Y - \mathbb{E}[\hat{\tau}^S_Y | ] )^2 |  \phi(\x, \Z) \right] \\
    &=  Cov(\T_W^T\Z | \phi(\X, \Z)) \T_W \\
    &=   Cov(\beta^T \X_W^T\Z| \phi(\X, \Z))  +  Cov(\R_W^T\Z| \phi(\X, \Z))  + 2  Cov(\beta^T \X_W^T\Z, \R_W^T\Z| \phi(\X, \Z)) \\ &\text{ using the decomposition in \cite{harshaw2019balancing}} 
\end{align}


The first term is the covariance of the truncated distribution of $\X_W^T \Z$. $\X_W^T \Z$. Since $X_W^T \Z$ is normal, by theorem 3.1 from ~\cite{rubin2011causal}:
\begin{align}
    Cov( \X_W^T \Z |  \phi(\X, \Z) ) = \frac{P(\chi^2_{k+2} \le a)}{P(\chi^2_k \le a)} Cov(\X_W^T \Z) 
\end{align}

% The third term: 
% \begin{align}
%     &Cov(\beta^T \X_W^T\Z, \R_W^T \Z |  \phi(\X, \Z) ) \\
%     &= \EE[ \beta^T \X_W^T \Z \Z^T \R_W |  \phi(\X, \Z) ] - \EE[\beta^T \X_W^T \Z |  \phi(\X, \Z) ] \EE[ \Z^T \R_W |  \phi(\X, \Z) ] \\
%     &= \EE[ \beta^T \X_W^T \Z \Z^T \R_W |  \phi(\X, \Z) ] - \EE[\EE[\beta^T \x_W^T \Z |  \phi(\X, \Z) ] |\X = \x, \phi] \EE[ \Z^T \R_W |  \phi(\X, \Z) ] \\
%     &= \EE[ \beta^T \X_W^T \Z \Z^T \R_W |  \phi(\X, \Z) ] - \EE[0 |\X = \x, \phi] \EE[ \Z^T \R_W |  \phi(\X, \Z) ] \text{because $\EE[\Z | \X = \x, \phi] = 0$}\\
%      &= \EE[ \beta^T \X_W^T \Z \Z^T \R_W |  \phi(\X, \Z)]  \\
%      &=\sum_i \sum_j \EE[\alpha_i Z_i Z_j R_j |  \phi(\X, \Z)] \text{where $\alpha^T = \beta^T \X_W^T$} \\
%      &= \sum_i \EE[\alpha_i 1 R_i|  \phi(\X, \Z)] + \sum_{i \neq j} \EE[\alpha_i Z_i Z_j |  \phi(\X, \Z)] \EE[R_j|  \phi(\X, \Z)] \\&\text{ because $Z_i^2 = 1$ and $R_j$ is independent of $X_i$ and $Z_i, Z_j$ when $i \neq j$} \\
%      &=0 \text{ because $\EE[X_i R_i] = 0$ and $\EE[R_i] =0$}
% \end{align}

For the second term, we first note that $U = ( \X_W^T \Z, \R_W^T \Z) = ( \X_W^T, \R_W^T) \Z $ is multivariate normal. 
 Since $ Cov( \R_W^T \Z,  \beta^T \x_W^T \Z ) = 0$, $\R_W^T \Z$ and $\X_W^T \Z$ are uncorrelated. Since $(\R_W^T \Z, \X_W^T \Z)$ is a multivariate normal and $\R_W^T \Z$ and $\X_W^T \Z$ are uncorrelated,  $\R_W^T \Z$ and $\X_W^T \Z$ are independent so $\R_W^T \Z$ is independent of $\phi(\X, \Z)$:
\begin{align}
    Cov(\R_W^T \Z| \phi(\x, \Z)) = Cov(\X_W^T \Z) 
\end{align}

For the 3rd term, since $\X_W^T \Z$ and $\R_W^T$ are independent and $\phi$ is a function of only $\X_W^T \Z$, $\X_W^T \Z$ and $\R_W^T$ are independent conditioning on $\phi$. Therefore: 
\begin{align}
    Cov(\beta^T \X_W^T\Z, \R_W^T\Z| \phi(\X, \Z)) = 0
\end{align}
Therefore:
\begin{align}
    \var_S(\hat{\tau}^S_Y | \phi(\X, \Z)) =\frac{P(\chi^2_{k+2} \le a)}{P(\chi^2_k \le a)} \beta^T Cov(\X_W^T \Z) \beta + Cov(\R_W^T \Z) 
\end{align}

\end{proof}

==> variance_linear.tex <==
\subsection{Variance - Linear}
We assume that $n_1 = n_0 = n/2$. First we add a bias term $1$ to the end of $x_1, .., x_n$ so that $x_i$ has dimension $d+1$. 
Define 
\begin{align}
    T_i &= \frac{Y_i^1 + Y_i^0}{2}
\end{align}

We assume that $T$ is linear in term of $X$: 
\begin{align}
    T = \beta^T X + R 
\end{align}
where $R$ is independent of $X$, and $\EE[R | \x] = \EE[R ]=0$. Let $\sigma_R^2 = Var(R)$.




Let $Z_i = 2A_i - 1 \in \{-1, 1\}$. Let $\X_W$, $\T_W$ and $\R_W$ denote the matrices $\X$, $\T$ and $\R$ where each row corresponding to data point $i$ is multiplied by $W_i$.
Let 
\begin{align}
\varphi(\x, \A) = \Z^T \x_w   [Cov(x_w^T \Z)]^{-1} \x_w^T \Z< a
\end{align}
be the balancing condition where
\begin{align}
    Cov(x_w^T \Z) 
    &= \EE[ x_w^T \Z \Z^T x_w] - \EE[x_w^T \Z] \EE[x_w^T \Z]^T\\
    &= x_w^T  \EE[ \Z \Z^T]x_w -  x_w^T \EE[ \Z] \EE[x_w^T \Z]^T \\
    &=   x_w^T  \EE[ \Z \Z^T]x_w \text{ because } \EE[ \Z] = \mathbf{0}
\end{align}
where since $\Z$ is the randomization design that make $n_0 = n_1$ we have $\EE[\Z \Z^T] = Cov(\Z) = (n\mathbf{I} - \mathbf{1}\mathbf{1}^T)/(n-1)$ with $\mathbf{I}$ being the identity matrix and $\mathbf{1}$ a vector of $\mathbf{1}$ (Section 3.2, page 8, \citep{harshaw2019balancing}). 

Therefore $\varphi(\x, \A)$ can be calculated by:
\begin{align}
\varphi(\x, \A) =  \frac{1}{n-1} \Z^T \x_w  [x_w^T  (n\mathbf{I} - \mathbf{1}\mathbf{1}^T) x_w]^{-1} \x_w^T \Z < a
\end{align}


First we note that
\begin{align}
    \varphi(\X, \A) = \varphi(\X, 1-\A)
\end{align}
which satisfies the condition in Lemma~\ref{lem:helper}. Let $\phi(\X, \Z)$ denote $\varphi(\X, \A)$




First we analyze the variance of $\hat{\tau}$ without the balance condition.
\begin{lemma}
\begin{align}
    \var_S(\hat{\tau}^S_Y | \x) = \frac{Cov_S(\frac{p_T(X)}{p_S(X)}X)}{n} + \frac{6\sigma_R^2}{n^2} \sum_{i=1}^n w_i^2
\end{align}
\end{lemma}
\begin{proof}
First we have:

\begin{align}
&\var_S(\hat{\tau}^S_Y | \x) \\
&= \EE \left[ \var_S(\hat{\tau}^S_Y | \x, \Y)  | \x \right] + \var( \EE_S[\hat{\tau}^S_Y | \x, \Y] |\x) \\
&= \EE \left[ \var_S(\hat{\tau}^S_Y | \x, \Y)  | \x \right] + \var\left( \frac{1}{n} \sum_{i=1}^n w_i (Y^1_i  - Y^0_i) | \x   \right) \\
&= \EE \left[ \var_S(\hat{\tau}^S_Y | \x, \Y) | \x \right] + \frac{1}{n^2} \sum_{i=1}^n w_i^2 \var (R^1_i  - R^0_i)  \\
&= \EE \left[ \var_S(\hat{\tau}^S_Y | \x, \Y) | \x \right] + \frac{2\sigma_R^2 \sum_{i=1}^n w_i^2 }{n^2} 
\end{align}

 For the first term:
\begin{align}
    &\frac{n^2}{4}\var_S(\hat{\tau}^S_Y | \x, \Y) \\
    &= \frac{n^2}{4} \EE \left[(\hat{\tau}^S_Y - \mathbb{E}[\hat{\tau}^S_Y | \x, \Y] )^2 | \x,\Y \right] \\
    &= \frac{n^2}{4} \T_w^T Cov(\Z) \T_w \\
    &=  \beta^T \x_w^T Cov(\Z) x_w \beta + \R_w^T Cov(\Z) \R_w + 2 \beta^T \x_w^T Cov(\Z) \R_w \text{ using the decomposition in \cite{harshaw2019balancing}}
\end{align}
Then 
\begin{align}
    &\frac{n^2}{4} \EE \left[ \var_S(\hat{\tau}^S_Y | \x, \Y) | \x \right] \\
    &=  \beta^T \x_w^T Cov(\Z) x_w \beta + \EE[\R_w^T Cov(\Z) \R_w | \x] + 2 \beta^T \x_w^T Cov(\Z)\EE[ \R_w | \x] \\
    &= \beta^T Cov( \x_w^T \Z) \beta+ \EE[\R_w^T Cov(\Z) \R_w | \x]\text{ because $\EE[ \R_w | \x] = 0$}
\end{align}
The first term $Cov(\x_w^T \Z)$ is the covariance of $\x_w^T \Z$. $\x_w^T \Z$ has a symmetric distribution and by finite population CLT \citep{li2016general}, when $n$ is large
$\frac{2}{n}\x_w^T \Z$ converges in distribution to $ Norm(0 , \frac{Cov_S(\frac{p_T(X)}{p_S(X)}X)}{n})$. 

The second term 
\begin{align}
\EE[\R_w^T Cov(\Z) \R_w | \x] = \sum_{i=1}^n \sum_{j=1}^n \EE[w_iR_i Cov(Z_i, Z_j) w_j R_j| \x]
\end{align}
When $i\ne\frac{p_T(X)}{p_S(X)}X j$ we can factor out $\EE[R_i | \x]$ because $R_i, R_j$ and $\Z$ are independent. Since $\EE[R_i | \x] = 0, ~\EE[w_iR_i Cov(Z_i, Z_j) w_j R_j]=0$ when $i \ne\frac{p_T(X)}{p_S(X)}X j$. Therefore:
\begin{align}
    &\EE[\R_w^T Cov(\Z) \R_w | \x] \\
    &= \sum_{i=1}^n w_i^2 \EE[R_i^2 \var(Z_i) | \x] \\
    &= \sum_{i=1}^n w_i^2 \EE[R_i^2] \var(Z_i) \\
    &= \sigma_R^2 \sum_{i=1}^n w_i^2 \text{ because } \EE[R_i^2]=\sigma_R^2 \text{ and } var(Z_i) = 1
\end{align}

Therefore:
\begin{align}
    &\var_S(\hat{\tau}^S_Y | \x) = \frac{Cov_S(\frac{p_T(X)}{p_S(X)}X)}{n} + \sigma_R^2 \frac{6}{n^2} \sum_{i=1}^n w_i^2
\end{align}
\end{proof}

Now we analyze the variance of $\hat{\tau}$ with the balance condition:
\begin{lemma}
Suppose $n_1 = n_0 = n/2$ and  $\x_w^T \Z$ has normal distribution (which is implied when $n$ is very large, using finite CLT \cite{li2016general}). 
Using the balance condition: 
\begin{align}
\varphi(\x, \A) = \phi(\x, \Z) =  x_w^T \Z [cov(x_w^T \Z)]^{-1} \Z^T  x_w  =  \frac{1}{n-1} x_W^T \Z [x_W^T  (n\mathbf{I} - \mathbf{1}\mathbf{1}^T) x_W]^{-1} \Z^T x_W < a
\end{align}
Then: 
\begin{align}
    \var_S(\hat{\tau}^S_Y | \x, \phi(\x, \Z)) =\frac{P(\chi^2_{k+2} \le a)}{P(\chi^2_k \le a)} \frac{Cov_S(\frac{p_T(X)}{p_S(X)}X)}{n} + \sigma_R^2 \frac{6}{n^2} \sum_{i=1}^n w_i^2
\end{align}
\end{lemma}
\begin{proof}

\begin{align}
&\var_S(\hat{\tau}^S_Y | \x, 
\phi(\x, \Z) ) \\
&= \EE \left[ \var_S(\hat{\tau}^S_Y | \x, \Y, \phi(\x, \Z))  | \x, \phi(\x, \Z) \right] + \var( \EE_S[\hat{\tau}^S_Y | \x, \Y, \phi(\x, \Z)] |\x, \phi(\x, \Z)) \\
&= \EE \left[ \var_S(\hat{\tau}^S_Y | \x, \Y, \phi(\x, \Z))  | \x, \phi(\x, \Z) \right] + \var\left( \frac{1}{n} \sum_{i=1}^n w_i (Y^1_i  - Y^0_i) | \x, \phi(\x, \Z)   \right) \\
&= \EE \left[ \var_S(\hat{\tau}^S_Y | \x, \Y, \phi(\x, \Z)) | \x, \phi(\x, \Z) \right] + \frac{1}{n^2} \sum_{i=1}^n w_i^2 \var (R^1_i  - R^0_i)  \\
&= \EE \left[ \var_S(\hat{\tau}^S_Y | \x, \Y, \phi(\x, \Z)) | \x , \phi(\x, \Z)\right] + \sigma_R^2 \frac{2 \sum_{i=1}^n w_i^2 }{n^2} 
\end{align}

For the first term:
\begin{lemma}
\label{lem:helper2}
\begin{align}
\EE \left[(\hat{\tau}^S_Y - \mathbb{E}[\hat{\tau}^S_Y | \x, \Y] )^2 | \x,\Y, \phi(\x, \Z) \right] 
    = \frac{n^2}{4} \T_w^T Cov(\Z | \phi(\x, \Z)) \T_w 
    \end{align}
\end{lemma}
\begin{proof}
Using Lemma A1 in \cite{harshaw2019balancing} we have: 
\begin{align}
    \hat{\tau}^S_Y - \mathbb{E}[\hat{\tau}^S_Y | \x, \Y] = \frac{2}{n} <\Z, \T_w>
\end{align}
Then:
\begin{align}
& \EE \left[(\hat{\tau}^S_Y - \mathbb{E}[\hat{\tau}^S_Y | \x, \Y] )^2 | \x,\Y, \phi(\x, \Z) \right] \\
&= \frac{4}{n^2} T_w^T \EE[ZZ^T | \x, \Y, \phi(\x, \Z)] T_w \\
&= \frac{4}{n^2} T_w^T \EE[ZZ^T |  \phi(\x, \Z)] T_w \\
    &= \frac{4}{n^2} \T_w^T Cov(\Z| \phi(\x, \Z)) \T_w \text{ because } \EE[\Z | \phi(\x, \Z) ] = 0 \text{ from Lemma~\ref{lem:helper}}
    \end{align}
\end{proof}
Using Lemma~\ref{lem:helper2}:
\begin{align}
    &\frac{n^2}{4}\var_S(\hat{\tau}^S_Y | \x, \Y, \phi(\x, \Z) ) \\
    &= \frac{n^2}{4} \EE \left[(\hat{\tau}^S_Y - \mathbb{E}[\hat{\tau}^S_Y | \x, \Y] )^2 | \x,\Y, \phi(\x, \Z) \right] \\
    &= \frac{n^2}{4} \T_w^T Cov(\Z | \phi(\x, \Z)) \T_w \\
    &=  \beta^T \x_w^T Cov(\Z| \phi(\x, \Z)) x_w \beta + \R_w^T Cov(\Z| \phi(\x, \Z)) \R_w + 2 \beta^T \x_w^T Cov(\Z| \phi(\x, \Z)) \R_w \\ &\text{ using the decomposition in \cite{harshaw2019balancing}}
\end{align}

Then 
\begin{align}
    &\frac{n^2}{4} \EE \left[ \var_S(\hat{\tau}^S_Y | \x, \Y, \phi(\x, \Z) ) | \x \right] \\
    &=  \beta^T \x_w^T Cov(\Z |  \phi(\x, \Z) ) x_w \beta + \EE[\R_w^T Cov(\Z |  \phi(\x, \Z) )) \R_w | \x] + 2 \beta^T \x_w^T Cov(\Z| \phi(\x, \Z) ))\EE[ \R_w | \x] \\
    &= \beta^T Cov( \x_w^T \Z |  \phi(\x, \Z) ) \beta+ \EE[\R_w^T Cov(\Z |  \phi(\x, \Z) ) \R_w | \x]\text{ because $\EE[ \R_w | \x] = 0$} \label{eq: decomposition}
\end{align}

The second term 
\begin{align}
\EE[\R_w^T Cov(\Z | \phi(\x, \Z) ) \R_w | \x] = \sum_{i=1}^n \sum_{j=1}^n \EE[w_iR_i Cov(Z_i, Z_j  | \phi(\x, \Z)) w_j R_j | \x]
\end{align}
When $i\ne\frac{p_T(X)}{p_S(X)}X j$ we can factor out $\EE[R_i | \x]$ because $R_i, R_j$ and $\Z$ are independent given $\x$. Since $\EE[R_i | \x] = 0, ~\EE[w_iR_i Cov(Z_i, Z_j) w_j R_j | \x]=0$ when $i \ne\frac{p_T(X)}{p_S(X)}X j$. Therefore:
\begin{align}
    &\EE[\R_w^T Cov(\Z | \phi(\x, \Z) ) \R_w | \x] \\
    &= \sum_{i=1}^n w_i^2 \EE[R_i^2 \var(Z_i | \phi(\x, \Z)) | \x] \\
    &= \sum_{i=1}^n w_i^2 \EE[R_i^2] \var(Z_i | \phi(\x, \Z)) \\
    &= \sum_{i=1}^n w_i^2 \text{ because } \EE[R_i^2]=\sigma_R^2 \text{ and } var(Z_i | \phi(\x, \Z) ) = \EE[Z_i^2 | \phi(\x, \Z)] - \EE[Z_i | \phi(\x, \Z)]^2 = 1 - 0 = 1
\end{align}

The first term $Cov(\x_w^T \Z)$ is the covariance of the truncated distribution of $\x_w^T \Z$. $\x_w^T \Z$ has a symmetric distribution and by finite population CLT \citep{li2016general}, when $n$ is large
$\frac{2}{n}\x_w^T \Z$ converges in distribution to $Norm(0 , \frac{Cov_S(\frac{p_T(X)}{p_S(X)}X)}{n})$. By theorem 3.1 from ~\cite{rubin2011causal}:
\begin{align}
    Cov( \x_w^T \Z |  \phi(\x, \Z) ) = \frac{P(\chi^2_{k+2} \le a)}{P(\chi^2_k \le a)} Cov(\x_w^T \Z) 
\end{align}

Therefore:
\begin{align}
    \var_S(\hat{\tau}^S_Y | \x, \phi(\x, \Z)) =\frac{P(\chi^2_{k+2} \le a)}{P(\chi^2_k \le a)} \frac{Cov_S(\frac{p_T(X)}{p_S(X)}X)}{n} + \sigma_R^2 \frac{6}{n^2} \sum_{i=1}^n w_i^2
\end{align}

\end{proof}



==> variance_linear_final.tex <==
\subsubsection{Variance Decomposition}
\label{sec:variance_linear}
In this section, we show the variance decomposition similar to \citep{harshaw2019balancing, kallus2018optimal} and use it to show the variance reduction achieved by balancing in Section~\ref{sec:variance_reduction}. We use this decomposition because it shows that the eigenvectors and the eigenvalues of the covariance matrix of the assignment vector are the main factors that affect the variance and variance reduction techniques. 
This is closely related to the concept of ``accidental bias'' of~\citet{efron1971forcing}, which is defined as the principal eigenvalue of the covariance of the assignment matrix.

We will generally consider an event, $\E$, to refer to a ``balance'' event.
In the case of re-randomization, this means that we condition on randomizations such that imbalance is below our specified criteria.
\begin{lemma}[minor changes to Lemma 1 in \citep{harshaw2019balancing}]
\label{lem:variance_decomposition_with_balancing}
For any event $\mathcal{E}$ such that $\EE[A_i | \E] = 1/2~ \forall i$:
\begin{align}
&\frac{n^2}{4} \var(\hat{\tau}^S_Y |  \x, \y, \E) \\
&= \ttt_w^T \EE[\Z \Z^T | \E]  \ttt_w \label{eq:var_decomp1}\\&= \beta^T  \EE[\x_w^T\Z \Z^T \x_w| \E]  \beta +   \rr_w^T \EE[\Z \Z^T| \E] \rr_w \\&      + 2 \beta^T \x_w^T\EE[\Z \Z^T| \E] \rr_w \label{eq:var_decomp2}
    \end{align}
\end{lemma}


For convenience, we recap  the intuition behind the variance decomposition in Lemma~\ref{lem:variance_decomposition_with_balancing} from \citep{harshaw2019balancing}. 

First we explain the term $\ttt_w^T \EE[\Z \Z^T | \E]  \ttt_w$ in Eq.~\ref{eq:var_decomp1}. The term shows that the eigenvectors and eigenvalues of $\EE[\Z\Z^T| \E]$ determine the variance as follows. Let $\e_1, ..., \e_n$ and $\lambda_1, .., \lambda_n$ be the normalized eigenvectors and corresponding eigenvalues of  matrix $\EE[\Z \Z^T | \E] $. Since $\EE[\Z\Z^T | \E]$ is symmetric, the eigenvectors form an orthonormal basis so we can write $\ttt_w$ as a linear combination of $\e_1, .., \e_n$ and get:
\begin{align*}
   \ttt_w = \norm{\ttt_w}\sum_{i=1}^n \eta_i \e_i 
\end{align*}
where $\eta_i = \langle \ttt_w, \e_i \rangle/\norm{\ttt_w}$ is the coefficient that captures the alignment of the weighted outcome $\ttt_w$ with respect to the eigenvector $\e_i$. 
Therefore:
\begin{align}
\label{eq:variance_eigenvector}
   \ttt_w^T \EE[\Z \Z^T | \E]  \ttt_w = \norm{\ttt_w}^2\sum_{i=1}^n \eta_i^2 \lambda_i
\end{align}
% and similarly:
% \begin{align*}
% \label{eq:variance_eigenvector2}
%   \ttt_w^T \EE[\Z \Z^T| \E]  \ttt_w = \norm{\ttt_w}^2\sum_{i=1}^m \eta_i'^2 \lambda_i'
% \end{align*}
% where $\e_1', ..., \e_m'$ and $\lambda_1', .., \lambda_m'$ be the normalized eigenvectors and corresponding eigenvalues of  matrix $\EE[\Z \Z^T | \E] $. 

Since $\eta_i^2> 0 ~\forall i$ and $\sum_{i=1}^n \eta_i^2  = 1$, Eq~\ref{eq:variance_eigenvector} shows that the variance can be written as a convex combination of the eigenvalues $\lambda_i$ of the covariance matrix of the assignment vector. To make this small, the weighted outcome $\ttt_w$ should be parallel to the eigenvector with the smallest $\lambda_i$, so that the smallest $\lambda_i$ is multiplied by the largest $\eta_i^2$. If we know $\ttt_w$, then we should choose balance event $\E$ such that $\ttt_w$ is parallel to the eigenvector with the smallest eigenvalue of $\EE[\Z\Z^T | \E]$. 

Since we do not know the weighted outcome $\ttt_w$ but can observe the weighted covariate $\x_w$, we decompose the weighted outcome $\ttt_w$  as
\begin{align}
\label{eq:t_decompose}
    \ttt_w = \x_w \beta  + \rr_w
\end{align}
where the first component demonstrates the predictive relationship of the covariates on the outcome. Substituting the decomposition of $\ttt_w$ in Eq.~\ref{eq:t_decompose} to Eq.~\ref{eq:var_decomp1} resulting in Eq.~\ref{eq:var_decomp2}. Since we know the covariates, we can reduce the first term in Eq.~\ref{eq:var_decomp2}. 

First we show that only the first term in Eq.~\ref{eq:var_decomp2} is affected by the balance event if the model is linear. Conditioned on $\x$, the second term is not affected by the balance event $\E$ and the third term is equal to $0$, resulting in the following lemma where only the first term is affected by the balance event $\E$: 

\begin{lemma}
\label{lem:variance_decomposition}
Let $n_1 = n_0 = n/2$. For any event $\E$ that only depends on $\X$ and $\Z$ and satisfies $\EE[ A_i | \E] = 1/2$:
    \begin{align*}
    \var_S(\hat{\tau}^S_Y | \x, \E) = \frac{4}{n^2}   \beta^T \EE[ \x_w^T\Z \Z^T \x_w| \E]  \beta + \frac{6}{n^2}\sigma^2_R \sum_{i=1}^n w_i^2 %\label{eq:variance_decomposition}
\end{align*}

\end{lemma}

This decomposition in Lemma.~\ref{lem:variance_decomposition} is useful because we can now use our knowledge of $\x_w$ to reduce the first term $\beta^T  \EE[\x_w^T\Z \Z^T \x_w| \E]  \beta$ and therefore reduce the variance. 
Since $\x_w^T\Z$ is asymptotically normal, $V= Cov(\x_w^T \Z)^{-1/2} \x_w^T\Z$ is asymptotically a standard multivariate normal distribution.  We express the variance in terms of $V$:

\begin{lemma}
\label{lem:variance_decomposition_normalized}
Let $n_1 = n_0 = n/2$. Let $V = Cov(\x_w^T \Z)^{-1/2} \x_w^T\Z$ and 
$\gamma^T = \beta^T Cov(\x_w^T \Z)^{-1/2}$. 
For any event $\E$ that only depends on $\X$ and $\Z$ and satisfies $\EE[ A_i | \E] = 1/2$:
    \begin{align}
    \var_S(\hat{\tau}^S_Y | \x, \E) = \frac{4}{n^2}   \gamma^T \EE[V V^T| \E ] \gamma + \frac{6}{n^2}\sigma^2_R \sum_{i=1}^n w_i^2 \label{eq:variance_decomposition_normalized}
\end{align}

\end{lemma}

Similar to Eq.~\ref{eq:variance_eigenvector}, the first term $ \gamma^T \EE[V V^T| \E ] \gamma$ is determined by the directions of $\gamma$ with respected to the eigenvectors of $\EE[VV^T | \E]$. Since we do not know $\gamma$, to make this quantity  small, we should choose the balance event $\E$ so that the largest eigenvalue of $\EE[VV^T| \E]$ is small, so that for any adversarial $\gamma$ the term  is small.  If $V$ is a standard multivariate normal distribution, all the eigenvalues of $V$ are the same and therefore an event $\E$ that reduces all the eigenvalues of $V$ equally will reduce the first term. 

\subsubsection{Variance Reduction}
\label{sec:variance_reduction}
In this section we will analyze the variance reduction achieved by Target Balance given in Definition~\ref{def:balance}. 



% \if0
% Consider the first term $\beta^T Cov( \x_w^T\Z | \phi) \beta$ in Eq.~\ref{eq: decomposition}. Define $V = Cov( \x_w^T\Z)^{-1/2} \x_w^T\Z$ and $\gamma^T = \beta^T Cov( \x_w^T\Z)^{-1/2}$ then we have:
% \begin{align*}
%     \beta^T Cov( \X^T\Z | \phi ) \beta = \gamma^T Cov(V | \phi) \gamma 
% \end{align*}
% where $Cov(V) = \I$

% Let $\e_1, ..., \e_m$ and $\lambda_1, .., \lambda_m$ be the eigenvectors and correspond eigenvalues of a matrix $\M$. Following \citep{harshaw2019balancing}, we write $\beta$ as a linear combination of $\e_1, .., \e_m$ and get:
% \begin{align*}
%   \gamma = \norm{\gamma}\sum_{i=1}^m \eta_i \e_i 
% \end{align*}
% where $\eta_i = <\gamma, \e_i>/\norm{\gamma}$. 
% Therefore:
% \begin{align*}
% \label{eq:eigen_decomposition}
%   \gamma^T \M \gamma = \norm{\beta}^2\sum_{i=1}^m \eta_i^2 \lambda_i
% \end{align*}
% Let $a_1, .., a_d$ denote the eigenvalues of $Cov(V | \phi)$. Since $Cov(V) = \I$, all eigenvalues of $Cov(V)$ is $1$. We will show that $\gamma^T Cov(V | \phi) \gamma  \le \gamma^T Cov(V ) \gamma $ by showing that $Cov(V| \phi)$ and $Cov(V)$ have the same eigenvectors, and $a_i \le 1 ~\forall 1 \le i \le d$
% \begin{lemma}
% \label{lem:ratio}
% $cov(V | \phi)$ is a diagonal matrix, where $a_i \le 1$ for all the diagonal entries $a_i$
% \end{lemma}
% \begin{proof}
% First we note that for any $u$ and $v$ such that $|u_i| = |v_i|~\forall 1 \le i \le d$, then $\PP(V = u) = \PP(V = v)$\my{ double check if it's true}. $\phi$ is equal to setting $\norm{V} < v_{\alpha}$ for some threshold $v_{\alpha}$
% The non-diagonal entry $(i,j)$ where $i \neq j$ of $Cov(V | \phi)$ is:
% \begin{align*}
%      & \sum_{\norm{v} \le v_{\alpha}} v_i v_j p(v)  \\
%       & = \sum_{\norm{v} \le v_{\alpha}} (v_i v_j + (-v_i) v_j+ v_i(-v_j)+ (-v_i)(-v_j)) \frac{p(v)}{4}  \\
%       &\text{ because $\PP(V = u) = \PP(V = v)$ for any $u$ and $v$ such that $|u_i| = |v_i|~\forall 1 \le i \le d$ } \\
%       &= \sum_{\norm{v} \le v_{\alpha}} 0 \frac{p(v)}{4} \\
%       &= 0 
% \end{align*}
% The diagonal entries $j$ is:

% \begin{align*}
%      & \sum_{\norm{v} \le v_{\alpha}} v_i^2 p(v)  \\
%      &\le \sum_{v} v_i^2 p(v)  \\
%      &=1 \text{ because $Cov(V) = \I$}
% \end{align*}
% \end{proof}

% \fi
Let $V = Cov(\x_w^T \Z )^{-1/2} \x_w^T\Z$. Recall that Target Balance is equal to:
\begin{align*}
\phi =
    \begin{cases}
      1, & \text{if}\ \norm{V}^2 < a \\
      0, & \text{otherwise}
    \end{cases}
\end{align*}

If $V$ is a standard multivariate normal distribution, Target Balance truncates $V$ spherically, so all the eigenvalues of the covariance matrix of $V$ are reduced.  Therefore for any $\gamma$, the term $\gamma^T \EE[V V^T| \E ] \gamma$ in Lemma~\ref{lem:variance_decomposition_normalized} is reduced. Theorem 3.1 from \cite{morgan2012rerandomization} shows the reduction ratio: 
\begin{lemma}[from the proof of Theorem 3.1 from \cite{morgan2012rerandomization}]
\label{lem:ratio}
If $W$ is a standard multivariate normal:
\begin{align*}
    \EE[W W^T| \norm{W}^2 < a]  = \frac{P(\chi^2_{d+2} \le a)}{P(\chi^2_d \le a)} \I%  \EE[V V^T]
\end{align*}
\end{lemma}

Therefore from Lemma~\ref{lem:variance_decomposition_normalized} and Lemma~\ref{lem:ratio} we can show if the weighted mean covariate is normal,  the variance with Target Balance is reduced compared to the variance without any balancing condition. Moreover in Section~\ref{sec:optimality} we will show that the reduction is optimal. 
 

\my{ add Condition 1 from \citep{li2018asymptotic} here}
\my{ add definition of the as-var}
By the finite population central limit theorem, 
\begin{align*}
    \hat{\tau}^S_Y | \x \xrightarrow[]{d} 
\end{align*}
\begin{theorem}
\label{thm:variance_with_balance}
Let $n_1 = n_0 = n/2$ and $\phi$ correspond to the balance condition in Definition~\ref{def:balance}. Let
$\gamma^T = \beta^T Cov(\x_w^T \Z)^{-1/2}$ and $\text{as-var}_S$ denote the variance  in the source of the asymptotic distribution. Then:%Let $V = Cov(\x_w^T \Z)^{-1/2} \x_w^T\Z$ and 
%$\gamma^T = \beta^T Cov(\x_w^T \Z)^{-1/2}$. Then:
\begin{align*}
    \text{as-var}_S(\hat{\tau}^S_Y | \x) =  \frac{4}{n^2} \gamma^T  \gamma +  \frac{6}{n^2}\sigma_R^2 \sum_{i=1}^n w_i^2\;.
\end{align*}
%If $\x_w^T\Z$ is a multivariate normal \footnote{Due to the finite central limit theorem, $\x_w^T\Z$ is asymptotically normal.}, then
\begin{align*}
    \text{as-var}_S(\hat{\tau}^S_Y | \x, \phi=1) = \frac{P(\chi^2_{d+2} \le a)}{P(\chi^2_d \le a)}  \frac{4}{n^2}   \gamma^T  \gamma + \frac{6}{n^2}\sigma^2_R\sum_{i=1}^n w_i^2 .
\end{align*}
\end{theorem}

Theorem~\ref{thm:variance_with_balance} shows that the variance can be decomposed into $2$ terms where the second term does not depend on the balance condition. The first term depends on the balance condition, and is reduced with Target Balance. 

\begin{corollary}
\label{thm:variance_with_balance}
Let $n_1 = n_0 = n/2$ and $\phi$ correspond to the balance condition in Definition~\ref{def:balance}.Then:
\begin{align*}
    &\text{as-var}_S(\hat{\tau}^S_Y ) \\ = & \frac{4}{n^2} \beta^T \EE_X Cov(X_W\Z)^{-1} \beta +  \frac{6}{n^2}\sigma_R^2 \sum_{i=1}^n w_i^2 \\
    & + \frac{1}{n} Var_S \left(\sum_{i=1}^n W_i \EE_S[Y^1_i -  Y^0_i | X] \right)\;.
\end{align*}
%If $\x_w^T\Z$ is a multivariate normal \footnote{Due to the finite central limit theorem, $\x_w^T\Z$ is asymptotically normal.}, then
\begin{align*}
&\text{as-var}_S(\hat{\tau}^S_Y | \phi = 1) \\ = &  \frac{P(\chi^2_{d+2} \le a)}{P(\chi^2_d \le a)}\frac{4}{n^2} \beta^T \EE_X Cov(X_W\Z)^{-1} \beta +  \frac{6}{n^2}\sigma_R^2 \sum_{i=1}^n w_i^2 \\
    & + \frac{1}{n} Var_S \left(\sum_{i=1}^n W_i \EE_S[Y^1_i -  Y^0_i | X] \right)\;.
\end{align*}
\end{corollary}

==> variance_simple.tex <==
\subsection{Variance - Simple Case}
We assume that $n_1 = n_0 = n/2$, $X \in R^d$ where $d=1$, and
\begin{align}
    Y^0_i = X_i + \epsilon^0_i \\
    Y^1_i = X_i + \beta + \epsilon^1_1
\end{align}
where $\beta$ is a constant and $\epsilon^0_i, \epsilon^1_i \sim Norm(0,1) $.

%Let $\bar{X_T} = \frac{2(\sum_{i: A_i = 1} X_i)}{n}$ and $\bar{X_C} = \frac{2(\sum_{i: A_i = 0} X_i)}{n}$ be the covariate means of the treated and control group. We also assume that $n$ is very large, and therefore $\bar{X_T}$ and $\bar{X_C}$ are normal $Norm(0,1)$. 

Let $\varphi(\X, \A) = \norm{ \frac{2}{n} \left( \sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} X_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  X_i\right) } < a$. First we note that:
\begin{align}
    \varphi(\X, \A) = \varphi(\X, 1-\A)
\end{align}
which satisfies the condition in Lemma~\ref{lem:unbiased2}. 

Let $Z = \frac{p_T(X)}{p_S(X)} Y^0$,  $Q = \frac{p_T(X)}{p_S(X)} X$ and $R = \frac{p_T(X)}{p_S(X)} \epsilon^0$.
\begin{align}
    \EE_S(Z) &= \EE_S\left(\frac{p_T(X)}{p_S(X)} Y^0 \right)  = \EE_T Y^0 = \EE_T X \\
    \EE_S(R) &= \EE_S \left(\frac{p_T(X)}{p_S(X)} \epsilon^0 \right) = \EE_T( \epsilon^0) = 0 \\
    \EE_S(Q) &= \EE_S \left(\frac{p_T(X)}{p_S(X)} X\right) = \EE_T(X)  
\end{align}
\begin{align}
    \var_S(Z) = \var_S\left(\frac{p_T(X)}{p_S(X)} Y^0 \right) 
    &= \EE_S \left(\frac{p_T(X)}{p_S(X)} Y^0  \right) ^2  - \left( \EE_S \frac{p_T(X)}{p_S(X)} Y^0 \right) ^2 \\
    &= \EE_T \left [\frac{p_T(X)}{p_S(X)} ({Y^0})^2\right ] - (\EE_T Y^0)^2 \\
    &= \EE_T \left [\frac{p_T(X)}{p_S(X)} ({Y^0})^2\right ] - (\EE_T X)^2
\end{align}
\begin{align}
    \var_S(Q) = \var_S\left(\frac{p_T(X)}{p_S(X)} X \right) 
    &= \EE_S \left(\frac{p_T(X)}{p_S(X)} X  \right) ^2  - \left( \EE_S \frac{p_T(X)}{p_S(X)} X \right) ^2 \\
    &= \EE_T \left [\frac{p_T(X)}{p_S(X)} (X)^2\right ] - (\EE_T X)^2 \\
    &= \EE_T \left [\frac{p_T(X)}{p_S(X)} (X)^2\right ] - (\EE_T X)^2
\end{align}
\begin{align}
     \var_S(R) = \var_S\left(\frac{p_T(X)}{p_S(X)} \epsilon^0 \right) 
    &= \EE_S \left(\frac{p_T(X)}{p_S(X)} \epsilon^0 \right) ^2  - \left( \EE_S \frac{p_T(X)}{p_S(X)} \epsilon^0 \right) ^2 \\
    &= \EE_T \left [\frac{p_T(X)}{p_S(X)} ({\epsilon^0})^2\right ] - (\EE_T \epsilon^0)^2 \\
    &= \EE_T \left [\frac{p_T(X)}{p_S(X)} ({\epsilon^0})^2\right ] \text{ because } \EE_T \epsilon^0 = 0\\
    &= \EE_T \left [\frac{p_T(X)}{p_S(X)} \right] \EE[ ({\epsilon^0})^2 ] \text{because  $\frac{p_T(X)}{p_S(X)}$ and $\epsilon^0$ are independent} \\
    &= \EE_T \left [\frac{p_T(X)}{p_S(X)} \right] \text{ because } \EE[ ({\epsilon^0})^2 ]=1
\end{align}
% \begin{align}
%     cov_S(Q,R) &= \EE_S[QR] - \EE_S[Q] \EE_S[R] \\
%     &= \EE_S\left[ \frac{p_T(X)^2}{p_S(X)^2} X \epsilon^0\right] - 0 
% \end{align}
First we analyze the variance of $\hat{\tau}$ without the balance condition:
\begin{align}
&\var_S(\hat{\tau} | \X= \mathbf{x}) \\
&= \frac{2}{n}\var_S(\frac{1}{n_1} \sum_{i=1}^n \frac{p_T(X_i)}{p_S(X_i)}A_i Y^1_i - \frac{1}{n_0} \sum_{i=1}^n \frac{p_T(X_i)}{p_S(X_i)} (1-A_i) Y^0_i | \X= \mathbf{x}) \\
&= \frac{2}{n}\var_S( \sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} Y^1_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  Y^0_i | \X= \mathbf{x}) \\
&= \frac{2}{n}\var_S( \sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} Y^0_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  Y^0_i | \X= \mathbf{x}) \\
&= \frac{2}{n}\var_S( \sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} X_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  X_i \big| \X= \mathbf{x}) \\&+ \frac{2}{n}\var_S( \sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} \epsilon^1_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  \epsilon^0_i \big| \X= \mathbf{x}) 
\end{align}
%Consider the first term. 
%Since $X_i \sim Norm(0,1)$, then:
% \begin{align}
%     \sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} X_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  X_i \sim Norm \left(0, \sum_{i=1}^n \left(\frac{p_T(X_i)}{p_S(X_i)} \right)^2 \right)
% \end{align}
The last equality is because conditioning on $\X = \mathbf{x}$, $\frac{p_T(X_i)}{p_S(X_i)}$'s are constants for all $i$, and therefore $ \sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} X_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  X_i $ and $\sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} \epsilon^1_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  \epsilon^0_i$ are uncorrelated. \my{ is this correct? } \anup{I think so. It is easier to see if we replace $\sum_{i: A_i=1}$ by $\sum_{i} A_i$ like in the first line. }

By finite population CLT \citep{li2016general}, $\frac{2}{n}( \sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} X_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  X_i ) | \X= \mathbf{x}$ converges in distribution to $Norm(0, \frac{\var_S(Q)}{n})$ and $\frac{2}{n}( \sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} \epsilon^0_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  \epsilon^0_i ) | \X= \mathbf{x}$ converges in distribution to $Norm(0, \frac{\var_S(R)}{n})$ when $n$ is large and \my{Is this correct?}.  Therefore when $n$ is large: 
\begin{align}
&\var_S(\hat{\tau}| \X= \mathbf{x}) = \frac{ \var_S(Q) +\var_S(R) }{n} 
\end{align}

Now we analyze the variance of $\hat{\tau}$ with the balance condition:
\begin{align}
&\var_S(\hat{\tau}| \X= \mathbf{x}, \varphi(\X, \A) = 1) \\
&= \frac{2}{n}\var_S(\frac{1}{n_1} \sum_{i=1}^n \frac{p_T(X_i)}{p_S(X_i)}A_i Y^1_i - \frac{1}{n_0} \sum_{i=1}^n \frac{p_T(X_i)}{p_S(X_i)} (1-A_i) Y^0_i | \X= \mathbf{x}, \varphi(\X, \A) = 1) \\
&= \frac{2}{n}\var_S( \sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} Y^1_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  Y^0_i \big| \X= \mathbf{x}, \varphi(\X, \A) = 1) \\
&= \frac{2}{n}\var_S( \sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} X_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  X_i \big| \X= \mathbf{x}, \varphi(\X, \A) = 1) \\&+ \frac{2}{n}\var_S( \sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} \epsilon^1_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  \epsilon^0_i \big| \X= \mathbf{x}, \varphi(\X, \A) = 1) 
\end{align}
The last equality is because conditioning on $\X = \mathbf{x}$, $\frac{p_T(X_i)}{p_S(X_i)}$'s are constants for all $i$, and therefore $ \sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} X_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  X_i $ and $\sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} \epsilon^1_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  \epsilon^0_i$ are uncorrelated. \my{ is this correct?}
% Consider the first term. Since $X_i \sim Norm(0,1)$, then:
% \begin{align}
%     \sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} X_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  X_i \sim Norm \left(0, \sum_{i=1}^n \left(\frac{p_T(X_i)}{p_S(X_i)} \right)^2 \right)
% \end{align}

We analyze the first term. Since $\frac{2}{n}( \sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} X_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  X_i \big| \X= \mathbf{x}$ is approximately $Norm(0, \frac{\var_S(Q)}{n})$ for large $n$, $\frac{2}{n}( \sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} X_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  X_i \big| \X= \mathbf{x}, \varphi(\X, \A) = 1$ is a truncated Gaussian. Let $V \sim Norm(0, \sigma^2)$, then $\var(V | \norm{V} < a)$ is: 
\begin{align}
    \sigma^2 \left[ 1- \frac{2\sqrt{a} g(\sqrt{a})}{F(\sqrt{a}/\sigma) - F(-\sqrt{a}/{\sigma})} \right]
\end{align}
where $g(x) = \frac{1}{\sqrt{2\pi}} exp(-0.5x^2)$ and $F(x)$ is the CDF of the standard normal distribution. Therefore the first term equal to:
\begin{align}
     \frac{var_S(Q)}{n} \left[ 1- \frac{2\sqrt{a} g(\sqrt{a})}{F(\sqrt{a}/\sigma) - F(-\sqrt{a}/{\sigma})} \right]
\end{align}

Now we analyze the 2nd term. Conditioning on $\X = \x$, $\frac{p_T(X_i)}{p_S(X_i)}$'s are constants for all $i$, therefore $\sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} X_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)} X_i$ and $\sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} \epsilon^1_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  \epsilon^0_i$ are independent \my{is it correct?}.  Therefore $\sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} \epsilon^1_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  \epsilon^0_i$ and $\varphi(\X, \A)$ are independent. 
\begin{align}
    &\frac{2}{n}\var( \sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} \epsilon^1_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  \epsilon^0_i \big| \X = \x, \varphi(\X, \A) = 1) \\
    = & \frac{2}{n}\var( \sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} \epsilon^1_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  \epsilon^0_i \big| \X = \x) 
\end{align}
By finite population CLT, $\frac{2}{n} (\sum_{i: A_i = 1} \frac{p_T(X_i)}{p_S(X_i)} \epsilon^1_i - \sum_{i: A_i = 0} \frac{p_T(X_i)}{p_S(X_i)}  \epsilon^0_i ) | \X = \x$ converges in distribution to $Norm(0, \frac{var_S(R)}{n}) $. Therefore the 2nd term is approximately $\frac{var_S(R)}{n}$ when $n$ is large. 

Summing up the first term and the second term:
\begin{align}
     &\var_S(\hat{\tau}| \X= \mathbf{x}, \varphi(\X, \A) = 1) \\
     &=\frac{var_S(Q)}{n} \left[ 1- \frac{2\sqrt{a} g(\sqrt{a})}{F(\sqrt{a}/\sigma) - F(-\sqrt{a}/{\sigma})} \right] + \frac{var_S(R)}{n}
\end{align}
Recall that: 
\begin{align}
&\var_S(\hat{\tau}| \X= \mathbf{x}) = \frac{ \var_S(Q) + \var_S(R) }{n} 
\end{align}

